Recovering Continuous Scene Dynamics from A Single Blurry Image with Events

This paper aims at demystifying a single motion-blurred image with events and revealing temporally continuous scene dynamics encrypted behind motion blurs. To achieve this end, an Implicit Video Function (IVF) is learned to represent a single motion blurred image with concurrent events, enabling the latent sharp image restoration of arbitrary timestamps in the range of imaging exposures. Specifically, a dual attention transformer is proposed to efficiently leverage merits from both modalities, i.e., the high temporal resolution of event features and the smoothness of image features, alleviating temporal ambiguities while suppressing the event noise. The proposed network is trained only with the supervision of ground-truth images of limited referenced timestamps. Motion- and texture-guided supervisions are employed simultaneously to enhance restorations of the non-referenced timestamps and improve the overall sharpness. Experiments on synthetic, semi-synthetic, and real-world datasets demonstrate that our proposed method outperforms state-of-the-art methods by a large margin in terms of both objective PSNR and SSIM measurements and subjective evaluations.

==> sec/1_introduction.tex <==


\IEEEraisesectionheading{\section{Introduction}\label{sec:introduction}}
\label{sec:intro}
% 

% 1. motion blurred图像中包含texture和motion信息，recover single image，丢失了motion信息，从而导致sequence的temporal ambiguity。xxx 和 xxx 利用sophestic的方法来消除temporal的ambiguity，
% 2. event数据提供了高帧率的intra-frame motion information，因此利用event可以帮助我们去进一步explore motion blurred image中的信息。EDI、LEDVDI、RED-Net、eSLNet等研究了如何利用event从motion blurred的图像中重建图像的过程。

% \IEEEPARstart{P}{erction} with the emergence of motion blur is a nuisance 
% deserves to be demystified to perceive the scene dynamics behind the blurred photographs~\cite{hqdeblurring_siggraph2008}. 
% Motion deblurring targets at , especially when encountering complex motions or severely blurred frames~\cite{zhang2021exposure}
% it is extremely challenging to achieve CTVB due to motion ambiguities and texture erasures caused by motion blurs~\cite{gupta2010single}. Furthermore, 

\IEEEPARstart{M}{otion} blur is a nuisance that commonly exists in photographs when perceiving scenes with relative motions from the camera to the targets~\cite{hqdeblurring_siggraph2008}. A real-world blurry image can be regarded as the integration of a continuous-time video, where the information on intra-frame motions and textures is missing~\cite{gupta2010single}. As the inversion of the blurry process, Continuous-Time {V}{ideo} extraction from a single Blurry image (CTVB) demystifies the motion blur by restoring the sharp latent image of arbitrary timestamps in the range of exposure time intervals, which allows us to see every subtle moment behind the blurry image, benefiting many real-world applications, \eg, sports photography, industrial monitoring, image segmentation, target tracking, and object recognition. %Nevertheless, CTVB is still 

% we have to explore motions or textures in  in restoring sharp latent images of arbitrary timestamps in the range of exposure time intervals requires either continuous. However, it is extremely challenging to achieve CTVB since 

% Compared with the conventional motion deblurring tasks, CTVB is more challenging. 
Different from CTVB, conventional frame-based motion deblurring approaches mostly focus on restoring a single image or a discrete-time video sequence. The ill-posedness is commonly relieved upon proper pre-defined priors/assumptions either on motions~\cite{krishnan2011blind,liu2020self,tai2011} or intensity textures~\cite{chen2019d,xu2013unnatural,fergus2006removing,pan2016blind}. Nevertheless, the performance of conventional approaches is confined 
to the above fragile assumptions. Even though the end-to-end learning networks based on the paired datasets can significantly improve the deblurring performance~\cite{gong2017motion,nimisha2017blur} and even achieve sequence restoration by decoupling the temporal motion ambiguity~\cite{purohit2019bringing,jin2018learning,rengarajan2020photosequencing}, the lack of continuous-time representations in terms of the intra-frame motions or textures hinders most existing frame-based approaches being applied for CTVB. 

Extraction of continuous-time representations of the intra-frame motions and textures from a single blurry image is generally difficult. Motion kernels~\cite{chen2019d,xu2013unnatural}, optical flows~\cite{chen2018reblur2deblur,liu2020self}, and exposure trajectories \cite{zhang2021exposure} are typical tools for continuous-time motion representations, which however often suffer from ill-posed nature of blur estimation. While the continuous-time texture representations are indirectly considered as the inter-frame consistencies between two consecutive blurry frames~\cite{jin2019learning}.
Nevertheless, it is still struggling to provide accurate estimations in terms of the missing motions and the erased textures during the whole exposure period, especially when encountering complex motions or severely blurred frames, and thus far from achieving CTVB. 



% To achieve CTVB, 

%  continuous time motion representation ~ Motion-ETR （Motion估计误差）
%  continuous time texture representation ~ E-CIR (polynomial引入一些误差，噪声会影响polynomial fitting，Motion缺失）、event-reshuffle（正反阈值会导致reveral的model与前向不同）
%  Motion + texture


% the frame-based methods have confined performance for general real-world scenarios, especially when encountering complex motions or severely blurred frames. 

% Nevertheless, the resulting algorithms largely rely on the domain-specific would suffer from performance degradation due to the violation of 
% existing frame-based methods a single \cite{pan2016blind,sun2013edge} or a sequence \cite{jin2018learning,purohit2019bringing,rengarajan2020photosequencing}


% to achieve the end 
% is an ill-posed problem due to the motion ambiguities and the texture erasures~\cite{gupta2010single}. Existing motion-deblurring approaches leverage artificial or data-driven priors to achieve the end but only a single \cite{pan2016blind,sun2013edge} or a sequence \cite{jin2018learning,purohit2019bringing,rengarajan2020photosequencing} of sharp latent images aligning to discrete timestamps can be restored, resulting in missing of crucial moments behind motion blurs, as shown in Fig.~\ref{fig:ivf_1}.

% Regarding the motions

% Regarding the textures

% Event-based approaches blabla ... 

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{fig/fig_method/fig1.png}
 \caption{Qualitative results of our proposed DeMo-IVF on the real-world dataset. An Implicit Video Function (IVF) is learned to represent a single blurry image with concurrent events. Using IVF, we query $109$ latent images from a single blurry image of different scenes, where {\it chr, cb}, and {\it st} respectively denote {\it chair, chessboard}, and {\it stool}, and we select the first $14$ frames for visualization.}
	\label{fig:ivf_1}
 \end{figure*}


% Even though motion blur largely degrades the quality of photos, 
% \IEEEPARstart{A}{companying} with the motion ambiguity and texture erasure, the motion blurs often exhibit mysteriously 
% the scene dynamics over time leads to motion blurs, accompanying the motion ambiguity and the texture erasure \cite{}. 
% Instead of a continuous-time video function, most existing approaches only recover a single \cite{pan2016blind,sun2013edge} or a sequence \cite{jin2018learning,purohit2019bringing,rengarajan2020photosequencing} of sharp latent images aligning to very limited timestamps, resulting in missing of crucial moments behind blurry images, \eg, xxx and xxx, as shown in Fig.~\ref{fig:overview}. 

% \IEEEPARstart{I}{ntegrating} the scene dynamics over time leads to motion blurs, a joint image degeneration accompanying the motion ambiguity and the texture erasure \cite{}. 
% Restoring a video sequence helps reveal the scene dynamics behind the blurry images 

% Most existing approaches focus on recovering a single \cite{pan2016blind,sun2013edge} or a sequence \cite{jin2018learning,purohit2019bringing,rengarajan2020photosequencing} of sharp latent images aligning to limited  timestamps that only reveals partial information behind motion blurs, resulting in the missing of crucial moments as shown in Fig.~\ref{fig:overview}. 

% two challenges: 1. ill-posedness of motion deblurring?
% 2. representation of continuous-time video function?

% To fully demystify the motion blurs, restoring sharp latent images of arbitrary timestamps during the exposure period is needed to reveal the temporally continuous scene dynamics.% and prevent missing crucial moments behind blurry images. 
% However, {m}{ost} of existing approaches only target at recovering a single \cite{pan2016blind,sun2013edge} or a sequence \cite{jin2018learning,purohit2019bringing,rengarajan2020photosequencing} of sharp latent images aligning to the limited discrete timestamps.

% by revealing the temporally continuous scene dynamics encrypted behind the blurry images is 

% is generally ill-posed since motions and textures are encrypted behind the blurry photographs \cite{jin2018learning,purohit2019bringing,rengarajan2020photosequencing}. Most of existing approaches focus on recovering a single latent image \cite{pan2016blind,sun2013edge} or a video sequence \cite{jin2018learning,purohit2019bringing,rengarajan2020photosequencing} of limited discrete timestamps

% \IEEEPARstart{M}{otion} blur is a nuisance which encrypts motions and textures behind the blurry photographs, resulting in ill-posedness when   sharp and clear scene dynamics generally ill-posed \cite{jin2018learning,purohit2019bringing,rengarajan2020photosequencing}  

% \textcolor{red}{Most of existing approaches focus on recovering a single latent image \cite{pan2016blind,sun2013edge} or a video sequence \cite{jin2018learning,purohit2019bringing,rengarajan2020photosequencing} that only reveals partial information behind motion blurs, resulting in the missing of crucial moments. Thus, the restoration of latent images at arbitrary timestamps is in need for real-world scenarios \cite{rozumnyia,jin2018learning}. }

% To fully demystify motion blurs, 
% \cite{pan2019bringing,pan2020high,wang2020event,xu2021motion,lin2020learning,jiang2020learning}

In this paper, we propose to employ the event camera to achieve CTVB, \ie, restoring the latent images of arbitrary timestamps as shown in Fig.~\ref{fig:ivf_1}. Different from the conventional frame-based cameras, event cameras perceive the scene dynamics by encoding brightness changes with extremely low latency (in the order of $\mu$s) and asynchronously emitting binary events with extremely high temporal resolution \cite{lichtsteiner128Times1282008,gallego2020event}. Thus events can provide intra-frame clues about motions \cite{zhu2018ev} and intensity textures \cite{rebecq2019c}, which bridges the gap between the blurry observations and the sharp latent images \cite{pan2019bringing}, unlocking the potential to reveal continuous-time scene dynamics behind blurry images. Many event-based motion deblurring approaches have recently been proposed and achieved prominent deblurring
performance even for complex motions or severely blurred frames~\cite{pan2020high,jiang2020learning,xu2021motion,wang2020event,zhang2022unifying,song2022cir,lin2020learning,shang2021bringing}. However, most of them~\cite{jiang2020learning,xu2021motion,lin2020learning,shang2021bringing} are dedicated to restoring a single image or a discrete-time video sequence instead of CTVB.

% Events convey intra-frame information on both motions and textures in a nearly continuous form, 
Similar to frame-based approaches, the performance of CTVB with events largely relies on the accuracy of continuous-time representations for the intra-frame motions and textures. 
% Recently, we have witnessed significant progress on event-based motion deblurring~\cite{pan2020high,jiang2020learning,xu2021motion,wang2020event,zhang2022unifying,song2022cir,lin2020learning,shang2021bringing}, but most existing approaches~\cite{jiang2020learning,xu2021motion,lin2020learning,shang2021bringing} are dedicated to restoring a single image or a discrete-time video sequence instead of CTVB. 
A sophisticated event reshuffle process~\cite{pan2020high,wang2020event,zhang2022unifying} is proposed as a time-dependent event representation to provide continuous-time texture compensations and finally achieve arbitrary-timestamp restorations. However, since the event thresholds are different between positive and negative polarities, the reshuffle process inevitably alternates event polarities and thus brings modeling errors~\cite{gallego2020event}. Meanwhile, parametric polynomials have been employed to approximate the per-pixel continuous-time intensity functions by fitting the temporal derivatives with events~\cite{song2022cir}, but the massive amount of event noise in spatial and temporal domains~\cite{inivaiton2020} would inevitably mislead the intensity polynomials, especially in static regions only with event noise. On the other hand, since instance optical flows would be predicted from events~\cite{zhu2018ev,wan2022learning}, CTVB can be fulfilled by warping latent restorations to any specific timestamps or turning to event-based video interpolation approaches~\cite{tulyakov2021time,tulyakov2022time,he2022timereplayer}. Nevertheless, the prediction error on optical flows and latent restorations can further be propagated to the final results. %\textcolor{red}{(ZX: how to validate the EV-Flow in our method does not suffer from the error propagation?)}

% However, to achieve this end, two main challenges still exist.

% Theoretically, one can recover latent sharp images of any timestamps providing reliable events \cite{scheerlinck2018continuous,pan2019bringing,Scheerlinck19ral,Wang21iccv}. However, t
% \begin{itemize}
    % \item {\bf Temporal Continuity.} 
    % One can achieve latent sharp image restoration of arbitrary timestamps \cite{scheerlinck2018continuous,pan2019bringing,Scheerlinck19ral,Wang21iccv} via a sophistical event reshuffle process \cite{pan2020high,wang2020event,zhang2022unifying}, which is however time-consuming and may suffer from temporal disturbances \cite{inivaiton2020}. While learning per-pixel parametric polynomials to represent videos \cite{song2022cir} would be computationally expensive for restoring latent images at subtle timestamps. %Thus, an efficient representation of the continuous-time video function is essential. 
    % \item {\bf Event Noise.} 
    
% The massive amount of event noise would inevitably contaminate the prediction of latent images and even produce worse results than conventional methods (without events) \cite{wang2020event,baldwin2020event,duan2021a}. Many learning-based approaches have been proposed \cite{xu2021motion,jiang2020learning} with the consideration of event noise suppression but for the purpose of restoring discrete-time image sequences. 
    % \cite{xu2021motion,jiang2020learning} or 
     % Thus, learning an efficient representation of the continuous-time video is another challenge. While parametric polynomial approximation \cite{song2022cir}  
% \end{itemize}
 %Thus event noise suppression . 
% ,baldwin2020event,duan2021a

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{fig/fig_method/fig_overview.png}
%  	\caption{}
% 	\label{fig:overview}
%  % \vspace{-2em}
% \end{figure}
% but they only focus on the restoration of a limited number of the latent images at fixed time instances, which raises the question: is it possible to learn a continuous-time video representation from a single blurry image with the concurrent events? 



% \paragraph{Event Noises} Although events properly bridge the blurry image and its latent images providing a naive model for continuous-time video representation. However, event noises are enormous both in spatial and temporal domains \cite{inivaiton2020}, which might be accumulated in EDI \cite{wang2020event}, resulting considerable image degradation \cite{pan2020high} especially in the static background. %Thus event noises cannot be negligible in the DeMo.%, but EDI model \eqref{eq:edi} 


% For the purpose of continuous-time video restoration, \ie, restoring the latent images at arbitrary time instances as shown in Fig.~\ref{fig:ivf_1}, 
Inspired by the implicit neural representation~\cite{mildenhall2020c}, we first bridge the gap between discrete-time and continuous-time video representations by learning an Implicit Video Function (IVF) from blurry images and events. It is more challenging than existing works using sharp and clear video clips \cite{Bemana2020xfields,benbarka2021,chen2021b,sitzmann2020,tancik2020}.
% This paper bridges the gap between discrete-time and continuous-time video representations for motion deblurring to restore the latent images at arbitrary time instances as shown in Fig.~\ref{fig:ivf_1}. Inspired by the implicit neural representation \cite{mildenhall2020c}, we propose to learn an Implicit Video Function (IVF) from blurry images and the concurrent events, which is more challenging than existing works (using sharp and clear video clips) \cite{Bemana2020xfields,benbarka2021,chen2021b,sitzmann2020,tancik2020}. 
To ease the burden, the overall architecture of the proposed IVF is divided into the temporally constant components, \ie, the blurry image, and the temporally alternating component, \ie, a continuous-time function closely related to events.
% (as a compensation). Then a continuous-time function to represent the alternating component which is closely related to events. 
For event noise, we mutually compensate events and frames to enhance the performance of IVF since the blurry image is less noisy than events while events are immune to motion blurs. 
% us to learn the IVF by mutual compensations. 
We employ the conditioned Multi-Layer Perceptrons (MLP) with the Fourier position encoding scheme to learn IVF and a dual feature embedding network (DFEN) to take the merits from both events and the blurry input in the feature domain. 
The overall network is only supervised by ground-truth images
of limited referenced timestamps. We further introduce motion- and texture-guided supervisions to enhance restorations of the non-referenced timestamps and improve the overall sharpness. 
% To validate the effectiveness of our proposed method, we implement experiments on both synthetic and real-world datasets.  
% with sharp and clear video inputs \cite{Bemana2020xfields}. 

% Inspired by the implicit neural representation (INR) \cite{mildenhall2020c}, a continuous-time video representation can be learned from clear and sharp video clips \cite{benbarka2021,chen2021b,sitzmann2020,tancik2020}.
% To enable the arbitrary timestamp motion deblurring, a continuous-time video representation should be learned. 

% The implicit neural representation (INR) provides 

% and largely relieve the motion ambiguities behind motion blurs \cite{xu2021motion}. However, the gap to the restoration of the latent image at arbitrary timestamps from a single blurry image still exists.


% Events emitted from event cameras  further demystify motion blurs with the help of  \cite{pan2019bringing,pan2020high,wang2020event}. 
% \paragraph{Blurry Images \vs Noisy Events} 

% \paragraph{Temporal Finity \vs Infinity} EDI is one of explicit functions, but 

%  有必要做任意时间插针的算法。但是存在两个挑战问题：
% 左右两针间隔很短，信号变化不大，噪声比较大，更有必要做互补融合
%  transformer
% 如何去学关于time的video implicit function？MLP+time encoding





% 
% Recently, event-based motion deblurring methods have been proposed to alleviate such ambiguities \cite{pan2019bringing,pan2020high,wang2020event,xu2021motion}, since events emitted from an event camera asynchronously encode the intra-frame latent motions and textures with extremely low latency \cite{gallego2020event}. 
% Due to the extremely low latency, events emitted from an event camera asynchronously encode the intra-frame latent motions and textures \cite{xu2021motion}. Hence, the illposedness of motion deblurring can be largely alleviated with events .







% Observing this point, we first investigate the {\color{red} uniqueness} of event-based motion deblurring problem. The theoretical result tells that {\color{red}xxxx}, the latent image functional (revealing temporally continuous video dynamics) can be uniquely determined if provided the concurrent events. 

% motivation
% 1。现有网络需要重新训练、或者需要额外的插针算法补充
% 2. 运动过大，现有网络还是存在missing的information






% % \lorem{1}
% % \input{fig/teaser}
% % \lorem{2}

% % 描述去模糊任务，基于event的去模糊，现有方法深度学习取得不错效果
% % 目前都是从ICCV中复制过来的
% % Due to motion ambiguities as well as the erasure of intensity textures, the task of motion deblurring is severely ill-posed. With the help of an event camera which can “continuously” emit events asynchronously with extremely low latency (in the order of µs), inherently embedding motions and textures, the task of motion deblurring can be essentially alleviated. 
% Recently, Many event-based motion deblurring methods have been proposed by learning from a large mount of data and achieved amazing results. 
% The used datasets are either built by synthesizing events with ESIM simulators on the existing deblurring datasets, or captured with event camera that simultaneously output events and APS frames.
% For synthesized datasets, Unable to consider some intricate noise in real scenes, tremendous discrepancy exists between the virtual events from event simulators and the real events emitted by event cameras. The datasets captured with event camera reflect real scenes more, but the output APS frames have low resolution and poor image quality , that cannot meet the needs of people's viewing and many applications, compared to frames shoot by RGB camera.
% % With the aid of EDI-based model or data-driven model, events can used to remove the blurred part of the image and obtain latent sharp images.
% % 但是这样的数据集有一定的限制
% % However, due to the limitations of bandwidth and technology, the blurry APS frames from event camera have low resolution and poor image quality. Sharp images obtained by removing blur from such APS frames still can not meet the needs of people's viewing and certain applications.
% % 融合不同相机的events和frames来解决该问题
% % The above problem can be solved by combing events and blurry images from extra RGB cameras to reconstruct high-quality, high resolution and high frame rate sharp images.
% To reconstruct higher quality clear video, a feasible solution is connecting event camera and RGB camera with a beam splitter to output low-latency event streams and high-quality intensity images for the same scene separately.
% % But as the camera settings change, new problems will also arise. Discrepancy in camera parameters like camera response function(CRF), resolution leads to the blur image and events output by two separate cameras does not fit the EDI model.
% % 对于该问题，以前的深度学习算法的问题
% The methods based on deep learning can utilize neural networks to learn the specific relationship from a large amount of data, but existing methods generally concatenate events and blur images and extract features with convolutional neural networks(CNNs), cannot complement and merge information well.
% % 我们解决该问题的方式
% In order to better extract and fuse features, we propose a new encoder with dual-branches architecture consisting of multi-stage hybrid CNN-Transformer architecture that can model long-range dependency and compensate each other between events and blurry images.

% % 现有的方法去模糊重建有限帧图像
% In addition, existing methods generally only reconstruct a fixed number of sharp images when using events for deblurring and do not make full use of the high time resolution characteristics of events. Theoretically, it is possible to reconstruct a sharp image video with a very high frame rate from the blur image with the aid of events. 
% Some methods first obtain sharp keyframes by deblurring and then interpolate other latent video frames from the initial deblurred images and events. However, solving the two problems sequentially causes a sub-optimal solution due to error accumulation.
% Recently the Local Implicit Image Function(LIIF) was proposed to represent images as a set of latent codes distributed in spatial dimensions and realized arbitrary super-resolution. 
% Inspired by that, we propose the Local Implicit Video Function(LIVF) for representing the latent sharp video from blurry images and events in a continuous manner. In LIVF, a video is represented as a set of latent codes distributed in spatial-temporal dimensions. Given the spatial coordinates and relative time, the decoding function queries the latent code at a corresponding position with a specified time to predict the intensity value. Since the time index is continuous, LIVF can be presented an arbitrary frame rate.

% 我们的方法（还没有想好网络名字）
% In this paper, we address the aforementioned problems by proposing the XXX network, which can remove the blur of images with events and reconstruct a sharp video with very high frame rate.
% The input of XXX is a blurry image and corresponding events that may come from different devices. XXX consists of three modules: (1)shallow feature extraction(SFE) module, (2)dense feature extraction and fusion module(DFEF), (3) decoding function module. 
% Specifically, the SFE module scales inputs to the same size by interpolation and extracts shallow features with CNN. 
% The DFEF module extracts deep features with residual dense blocks and complements information across events and images with swin-transformer layers in a multi-stage manner. 
% The extracted features represents latent 


The contributions of this paper are three-fold:
% \vspace{-1em}
\begin{itemize}
% \setlength\itemsep{-.3em}
\item We propose to learn an implicit video function from blurry images and the concurrent events, which fully {\it De}mystifies {\it Mo}tion blurred images (DeMo) and produces temporally continuous sharp sequences. To the best of our knowledge, this is the first work about learning an IVF from a single blurry frame and concurrent events. 
% Finally, we propose to fully {\it De}mystify {\it Mo}tion blurred images (DeMo) based on the learned IVF, \ie, DeMo-IVF.
% \vspace{-1em}
\item We propose a dual feature embedding network, \ie, DFEN, to simultaneously consider the event noise suppression and the blurry feature enhancement by multi-stage transformers. An Event-based Edge Refinement (EER) module is also presented to enhance the overall texture restoration performance.
% \vspace{-1em}
\item We propose to train the overall network with motion- and texture-guided supervisions only based on limited ground-truth images of limited referenced timestamps. We evaluate the DeMo-IVF on both synthetic and real-world datasets, showing that DeMo-IVF outperforms state-of-the-art methods in both restoration quality and temporal resolution. 
% Ideally, the proposed DeMo-IVF can restore $\infty$ frames from a single blurry image, thus fully demystifying motion blurs.
\end{itemize}



% In a nutshell, contributions of this paper are three-fold:
% % \vspace{-1em}
% \begin{itemize}
% % \setlength\itemsep{-.3em}
% \item We propose to learn an Implicit Video Function (IVF) from blurry images and concurrent events. To the best of our knowledge, this is the first work about learning an IVF from blurry and noisy inputs. Finally, we propose to fully {\it De}mystify {\it Mo}tion blurred images (DeMo) based on the learned IVF, \ie, DeMo-IVF.
% % \vspace{-1em}
% \item We propose a Dual Feature Embedding Network (DFEN) to simultaneously consider the event noise suppression and the blurry feature enhancement by multi-stage transformers.
% % \vspace{-1em}
% \item We evaluate the DeMo-IVF on both synthetic and real-world datasets, showing that DeMo-IVF outperforms state-of-the-art methods in restoration quality and temporal resolution. Ideally, the proposed DeMo-IVF can restore $\infty$ frames from a single blurry image, thus fully demystifying motion blurs.
% \end{itemize}

==> sec/2_related.tex <==
\section{Related Work}
\label{sec:related}

% \AT{introduce subtopics, mention surveys here}
% \lorem{1}

 %< bloody latex and its heuristics for figure placement

% \paragraph{Motion Deblurring}
% Motion blur commonly happens with moving objects during the exposure period, leading to visual degeneration and inherently encodes motions and textures in captured blurry images \cite{jin2018learning}. 
\noindent \textbf{Motion Deblurring.}
The task of motion deblurring aims to restore sharp clear latent images and reveal the hidden information behind motion blurs which, however, is generally ill-posed. We can roughly categorize existing approaches into {\it single image} and {\it video sequence} according to the number of restored image frames.
For the single image restoration,  early attempts of optimization-based methods generally require properly pre-defined priors/assumptions either on motions or on intensity textures, \eg, linearity \cite{liu2020self} and projective motion path \cite{tai2011} is often assumed for motions, and priors like gradient prior \cite{chen2019d}, sparsity \cite{xu2013unnatural,hu2010}, Gaussian scale mixture \cite{fergus2006removing} and dark channel \cite{pan2016blind} are exploited for intensity textures. 
However, identifying a suitably informative and general prior is difficult and crucial for the deblurring performance, and improper priors may lead to artifacts and degraded results \cite{zhou2019spatio}.
% However, identifying a suitably informative and general prior for motion blurs is struggling, while improper prior may even generate artifacts and degrade deblurring performance \cite{zhou2019spatio}.
To overcome the limitations of manual priors, learning-based methods leverage the merits of convolutional neural networks (CNNs) to predict latent sharp images in an end-to-end manner, achieving prominent performance \cite{gong2017motion,nimisha2017blur}. However, single-image restoration reveals only the static intensity textures but loses the entire motion information behind the blurry image.  
% scene dynamics, which is an important message behind motion blurs.

% The {\bf $\mathbf{1}$-to-many} motion deblurring methods restore a video sequence and reveal the scene dynamics, 
Existing video sequence restoration methods reveal the scene dynamics by extracting a predefined fixed number of latent images from one blurry frame, where the temporal ambiguity is one of the critical challenges \cite{zhang2021exposure,zhang2020g,jin2018learning,jin2019learning,purohit2019bringing,rengarajan2020photosequencing}. Constraints of temporal ordering \cite{jin2018learning,purohit2019bringing} and motion consistency \cite{zhang2021c,zhang2020g} have been investigated to decouple such temporal ambiguity. On the other hand, the inter-frame consistency has also been exploited to learn time ordering from two consecutive blurry images \cite{jin2019learning} or clear images (with short exposure time but noisy) \cite{rengarajan2020photosequencing}. 
% However, to the best of our knowledge, existing approaches only focus on the task of motion deblurring with a fixed number of reconstructions, which cannot be directly employed to restore the latent sharp images of arbitrary timestamps, resulting in the missing of crucial moments \cite{rozumnyia}. (\textcolor{red}{contradict with sec 5.2})
Despite these efforts, the frame-only approaches still struggle in sequence restoration, especially when the motion blur is large. 
Without additional auxiliary signal input, arbitrary frame reconstruction is even more unattainable.
    
% cycle flow consistency \cite{zhang2020g}, motion offset with linear / quadratic motion constraint \cite{zhang2021c}
% {\color{red} Jin \etal pioneer to recover a sequence of sharp frames from a single motion-blurred image~\cite{jin2018learning}, where they sequentially train multiple neural networks with a temporal invariant loss. Purohit \etal utilize a single recurrent neural network to generate the entire sequence~\cite{purohit2019bringing} which, however, may suffer from ambiguities in temporal ordering. Take this into account, Jin \etal tackle the problem of the temporal ambiguity by feeding multiple motion blurred images~\cite{jin2019learning}, while Rengarajan \etal additionally use two consecutive images over a short exposure time \cite{rengarajan2020photosequencing}.}

% Early attempts address this problem by assuming spatially uniform motion where blurs can be modelled as the convolution of a blur kernel with a sharp latent image, leading to the kernel-based motion deblurring approaches by means of regularized deconvolution \cite{krishnan2011blind,sun2013edge}.  Thus it enables the possibility of motion deblurring for visualization of the dynamic scene behind blurred photographs \cite{jin2018learning,jin2019learning,purohit2019bringing}. 

% 连续帧重建？
% 现有方法都是只重建1帧或者多帧，而且大多数学习的方法只能学到从单个blur图像到固定index的映射。多帧的重建逐渐成为deblur问题的热点，因为多帧能更好的反映blur内图像的动态过程，帮助我们清晰的理解场景。但是，相比单帧的重建问题，多帧的重建更为复杂，因为temporal ambiguity。xxx论文通过order loss解决了这个问题。另外一种解决该问题的方法是利用前后blur帧，得到的光流约束来解决temporal ambiguity。但是上述方法都只能重建有限的帧的重建，
% 如果需要得到其他帧率的结果，
% 要么需要重新训练，那么就耗费时间，而且不太实际
% 或者通过interpolation网络进一步插值，那么需要满足插值算法的运动场假设
% 
% detail-aware networks to refine subtle motion between continuous frames using Gram Matrix.... only reconstruct 7 frames
% To the best of our knowledge, 还没有工作直接从单帧blur图像中重建任意时刻的清晰图像，这在实际应用中非常有用。




% \paragraph{Event-Based Motion Deblurring}
\noindent \textbf{Event-based Motion Deblurring.}
Benefiting from the extremely high temporal resolution, events can provide the missing intra-frame information about motions and intensity textures \cite{lichtsteiner128Times1282008}. Hence, the gap between the blurry observations and the latent sharp images can be potentially bridged \cite{pan2019bringing}. According to the physical model of event cameras \cite{gallego2020event}, explicit relations are built between events and images. Many continuous-time event-based motion deblurring algorithms are proposed such as the complementary filter \cite{scheerlinck2018continuous}, the event-based double integral (EDI) \cite{pan2019bringing}, the asynchronous spatial convolution \cite{Scheerlinck19ral}, and the asynchronous Kalman filter \cite{Wang21iccv}.
% As pioneer efforts, the complementary filter \cite{scheerlinck2018continuous}, the event-based double integral (EDI) \cite{pan2019bringing}, the asynchronous spatial convolution \cite{Scheerlinck19ral} and the asynchronous Kalman filter \cite{Wang21iccv} have been proposed for motion deblurring and high frame rate video reconstruction. According to the physical model of event cameras \cite{gallego2020event}, explicit relations are built between events and images resulting in continuous-time event-based motion deblurring algorithms. 
However, the ideal model of event generation is often disturbed in real-world scenarios due to the huge amount of noise caused by the imperfection of physical circuits \cite{inivaiton2020}, leading to performance degradation in practice \cite{scheerlinck2018continuous}. 


% Compared to these model-based approaches, learning-based methods effectively suppress noise by fitting the distribution of noisy events \cite{wang2020event,wang2020joint,lin2020learning,xu2021motion}. eSL-Net is proposed to deal with event noise by leveraging the sparsity behind latent images \cite{wang2020event}, but it may result in over-smoothness due to the inconsistency between the synthetic events (for training) and the real-world events (for inference). LEDVDI tackles such inconsistency by training directly on real-world events \cite{lin2020learning}, and RED-Net further improves the deblurring performance by training the network with both synthetic and real-world events in a semi-supervised manner \cite{xu2021motion}. However, existing learning-based approaches with events only focus on restoring the latent images at pre-defined timestamps and a re-training phase or a cascaded interpolation network is required to enable reconstruction at arbitrary time instances.
Compared to these model-based approaches, learning-based approaches effectively suppress noise by fitting the distribution of noisy events \cite{wang2020event,wang2020joint,lin2020learning,xu2021motion}. 
Jiang \etal \cite{jiang2020learning} reinterpret a sequential deblurring process by a convolutional recurrent neural network.
Lin \etal \cite{lin2020learning} use events to estimate the residuals of deblurring and interpolation for sharp frame restoration, and they propose to use a dynamic filtering layer to handle spatially varying triggering thresholds for events.  
Xu \etal \cite{xu2021motion} exploit photometric consistency and blurry consistency to train the network with both synthetic and real-world data in a semi-supervised manner to bridge the gap between simulated and real-world motion blurs. 
% D2Net
Shang \etal \cite{shang2021bringing} assume that sharp frames usually appear nearby blurry frames and propose a principled framework for tackling video deblurring with non-consecutively blurry frames.
% EVDI
However, these approaches only focus on restoring the latent images at pre-defined timestamps and a re-training phase or a cascaded interpolation algorithm is required to enable reconstruction at arbitrary time instances.
Based on the event-enhanced degeneration model, Wang \etal \cite{wang2020event} propose a sparse learning framework to accomplish high-quality image reconstruction. By reorganizing the inputs, \ie, splitting the events and then reversing the order and polarity of the previous segment events, it is able to control which moment of the sharp image is reconstructed. 
But this method requires modifying the input and re-inferring for reconstruction at each timestamp, which is less efficient. In addition, the effect of temporal perturbations on events may be amplified.
Song \etal \cite{song2022cir} propose to predict sharp videos represented by the per-pixel parametric polynomials that also support infinitely high frame rate reconstruction. In order to train such a model, it is required to fit polynomial coefficients as supervision signals using the least squares method, which is time-consuming because a sufficient number of sharp images must be available to guarantee the fitting accuracy.

% achieve the {\bf $\mathbf{1}$-to-$\infty$} motion deblur.

% 基于事件相机的deblur？
% 事件相机输出高时间分辨率的事件点，从中可以发掘motion和texture的线索，进一步减轻deblur的难度。xxxx论文建立了event，blur和laent image之间的关系，得到了explict的deblur算法。但是，EDI仅仅通过pixel wise的event累计，对blur图像进行补偿从而得到latent image，对噪声极为敏感。 pan1，pan2，accv cedric，根据物理模型推导了连续时间事件重建模型，可以得到任意时刻的latent image的重建，但是由于事件数据非常噪声大，重建结果不太好。kalman模型xxxx需要引用。相比于deep learning的方法，model based的方法对噪声的怒棒性较差，因此基于神经网络的任意（连续时间）delbur方法可以有效解决噪声的问题，但是目前还没有相关工作。

% 在神经网络的方法方面。Wang的工作针对EDI的噪声问题，基于稀疏学习提出了xxxx网络，但是通过仿真的event训练网络，可能导致数据不匹配，从而在真实数据上over smoothness的问题。LEDVDI和徐芳的工作，利用真实event进行监督/半监督训练，得到了1-to-many的deblur网络，改善了在真实数据上的deblur性能。但是，目前所有的方法都是1-to-many的deblur网络，同传统图像的deblur网络一样，如果要xxx，需要重新训练，或者利用interpolation网络进行插值，这样不太贴合实际。

% 隐神经函数INF
% Directly学习从时间到pixel的映射是一个思路。在INF领域中，从location 到 rendering，从time到audio，从location+time到video，都有人研究。position encoding提高图像的细节描述，Fourier的encoding方法，bla。。。上述研究的都是从high quality的数据中学习INF
% 那么，而当data本身是降质的blur图像，如何从blur中学到location+time到video的INF也是一个相当困难的事情。

% 我们将联合事件，借助INF的思路，从而解决了这个问题。

% {\color{red} 

% Data driven algorithms relax the above limitations by utilizing  neural networks and directly learn the relation from a blurry image to a sequence of sharp clear images with the aid of events \cite{lin2020learning,wang2020event,jiang2020learning}. For training purpose, a synthesized dataset composed of labeled events and blurry images is commonly simulated from sharp clear video sequences \cite{jiang2020learning,wang2020event} which, however, may have inconsistency to the real events due to event noise in the spatio-temporal domain. Even though data variations have been considered by manually adding noise \cite{wang2020event,stoffregen2020reducing}, the generalizability remains limited for real event cameras. 
%   }

% Most of existing approaches aim at recovering its discrete version ${\bf I}_n \triangleq {\bf I}(t_n)$ with $n$ denoting the index of timestamp $t_n\in \mathcal{T}$. And the restoration of latent clear images requires to assume linear or piece-wise linear motion during the exposure interval which is however not applicable in many realistic scenarios, \eg, with non-rigid moving objects or under complex scenes. 

% for  further improving the temporal resolution, the temporal ambiguities \cite{jin2018learning} or requiring an additional interpolation network \cite{jin2019learning}. 
% \cite{acne}
% \lorem{2}
% 1. single frame restoration
% 2. sequence / video restoration
% 3. arbitrary sequence restoration ... inter
%  Jin (flawless slow motion) proposed deblurNet + interpNet, two blurry frames are required
% 

% \paragraph{Event-based Motion Deblurring}
% \cite{nasa}
% \lorem{2}

% \paragraph{Implicit Neural Representation}
\noindent\textbf{Implicit Neural Representation.}
% \cite{bspnet}
% \lorem{2}
Our work is related to the implicit neural representation (INR), which approximates the continuous functions that map the domain of the input signal (coordinates, time, voxel, \etc) to a representation of color, amplitude, or density at an arbitrary input location \cite{benbarka2021,chen2021b,sitzmann2020,tancik2020}. The idea of learning the INR with multi-layer perceptrons has been widely applied in various fields such as 3D rendering \cite{mildenhall2020c}, video generation \cite{niemeyer2019}, and image representation \cite{chen2021b}. Considering the motion deblurring task with continuous time instances, we cast it as learning an implicit video function (IVF) from a blurry image. Unlike existing approaches \cite{niemeyer2019,mildenhall2020c,pumarola2020,tretschk2021} that aim to learn an IVF from multi-view sharp and clear images, our task directly accepts motion-blurred input which is more challenging.  


==> sec/3_method.tex <==
\input{fig/fig_ivf_1.tex}
\begin{figure*}[!th]
\centering
\includegraphics[width=1\textwidth]{fig/fig_method/ivf_network2.jpg}
\caption{Architecture of the proposed DeMo-IVF, which is composed of the Dual Feature Embedding Network (DFEN) and the Continuous-time Decoding MLP. A single blurry image and the concurrent events are separately processed in DFEN by multi-layer transformers with the dual attention mechanism for event noise suppression and blurry feature enhancement. Then the latent sharp images at the arbitrary timestamp $t$ are restored by the continuous-time decoding MLP. }
%\textcolor{red}{(ZX: do we need to depict EER in this figure?)}}
\label{fig:overview_dals}
\end{figure*}
% \section{Problem Statement}
\section{Method}

\subsection{Problem Formulation}
Physically, a motion-blurred image $\bf B ({\bf x})$ can be expressed as the average of latent images over the exposure period $\mathcal{T}$,
\begin{equation}\label{eq:blur}
{\bf B} ({\bf x}) = \frac{1}{|\mathcal{T}|}\int_{t\in \mathcal{T}} {\bf I}({\bf x},t) dt ,
\end{equation}
where the latent scene dynamics ${\bf I}({\bf x},t)$ is a continuous function mapping positions $\bf x$ and timestamps $t$ to pixel values\footnote{We drop $\bf x$ for simplification in the following.}. 
Given a finite index set $\mathcal{N} \subset \mathbb{Z}$, restoring the $n$-th latent sharp image ${\bf I}_n, n\in \mathcal{N}$ of the continuous scene dynamics ${\bf I}(t)$ from the blurry image $\bf B$ is an ill-posed problem \cite{jin2018learning,purohit2019bringing,rengarajan2020photosequencing}.
Many algorithms have been proposed but only for the restoration of discrete version of ${\bf I}(t)$, \ie, ${\bf I}_n$ corresponding to the latent clear image at time $t_n\in \mathcal{T}$, through event-based motion deblurring networks (denoted as EMD-Net)\cite{lin2020learning,jiang2020learning,wang2020event,xu2021motion}.
\begin{equation}\label{eq:deblurNet}
    \{{\bf I}_n\} = \mbox{EMD-Net}({\bf B}, \mathcal{E}_{\mathcal{T}}),
\end{equation} 
where $\mathcal{E}_{\mathcal{T}} \triangleq \{({\bf x}_i,p_i,t_i)\}_{t_i\in \mathcal{T}}$ is the set of events triggered in $\mathcal{T}$ with $t_i$ and ${\bf x}_i$ respectively denoting the timestamp and the pixel location of the $i$-th event, and $p_i\in \{+1,-1\}$ denoting the polarity. $\text{EMD-Net}(\cdot)$ is a sequence reconstruction operator, and once it has been trained, only the latent clear images of fixed timestamps $t_n$ can be predicted. Thus, an interpolation algorithm is often required to restore the latent images off the fixed timestamps \cite{lin2020learning}, which increases the complexity and even results in sub-optimal solutions due to the propagation of deblurring errors.


In this paper, we target fully {\it De}mystifying {\it Mo}tion-blurred images (DeMo) with events by directly recovering the temporally continuous scene dynamics ${\bf I}(t)$ behind motion blurs. 
Different from Eq. \eqref{eq:deblurNet}, the task of DeMo is to restore sharp latent images of any timestamp $t$ during the exposure time interval $\mathcal{T}$. It can be realized by learning an implicit neural representation, \ie,
%\cite{niemeyer2019,mildenhall2020c,pumarola2020,tretschk2021}
\begin{equation}\label{eq:demo}
    {\bf I}(t) = \mbox{DeMo}(t; {\bf B}, \mathcal{E}_{\mathcal{T}}), \forall t\in \mathcal{T},
\end{equation}
which is an implicit video function of time $t$ conditioned on a single blurry image $\bf B$ and the corresponding event stream $\mathcal{E}_{\mathcal{T}}$. Different from achieving the DeMo task in two stages, \ie, deblurring and temporal upsampling \cite{jin2018learning,purohit2019bringing}, we aim at learning the scene dynamics as an Implicit Video Function (IVF) from a blurry image and the concurrent events. The resulting IVF is temporally continuous and thus allows querying latent sharp images of any time within the exposure period $\mathcal{T}$. We consider the IVF as a combination of the temporally constant (TC) component, \ie, the blurry image $\bf B$, and the temporally alternating (TA) component, \ie, $\phi_\theta$,
\begin{equation}\label{eq:ivf}
    {\bf I}(t) = {\bf B} + \phi_\theta (t;f_\gamma\left({\bf B}, \mathcal{E}_{\mathcal{T}}\right)),
\end{equation}
where $f_\gamma$ is a feature embedding function (with $\gamma$ denoting the parameters) to encode temporal variations in the feature domain in a higher dimension, and $\phi_\theta$ is a decoding function parameterized by an MLP (with $\theta$ as its parameters) to restore the TA component. Both $\phi_\theta$ and $f_\gamma$ are shared for any blurry image ${\bf B}$ and  events $\mathcal{E}_{\mathcal{T}}$.


% In our setting, learning a DeMo operator faces two main challenges:
% Physically, a motion blurred image $\bf B ({\bf x})$ can be expressed as an average over the exposure period $\mathcal{T}$, \ie, 
% \begin{equation}\label{eq:blur}
% {\bf B} ({\bf x}) = \frac{1}{|\mathcal{T}|}\int_{t\in \mathcal{T}} {\bf I}({\bf x},t) dt ,
% \end{equation}
% where the latent scene dynamics ${\bf I}({\bf x},t)$ is a continuous function mapping positions and timestamps to pixel values\footnote{Without specification, $\bf x$ is dropped for simplification.}. Given a finite index set $\mathcal{N} \subset \mathbb{Z}$, restoring the $n$-th latent image ${\bf I}_n, n\in \mathcal{N}$ of the continuous scene dynamics ${\bf I}(t)$ from a single blurry image $\bf B$ is a sequence reconstruction problem, which has been addressed in literature \cite{jin2018learning,purohit2019bringing,rengarajan2020photosequencing}.
% In this paper, we target at fully {\it De}mystifying {\it Mo}tion-blurred images with events (DeMo) by directly recovering the temporally continuous scene dynamics ${\bf I}(t)$ behind motion blurs. Many algorithms have been proposed but only for restoration of discrete version of ${\bf I}(t)$, \ie, ${\bf I}_n$ corresponding to the $n$-th latent clear image at time $t_n\in \mathcal{T}$, through event-based motion deblurring networks (EMD-Net) \cite{lin2020learning,jiang2020learning,wang2020event,xu2021motion}.
% \begin{equation}\label{eq:deblurNet}
%     \{{\bf I}_n\}_n = \mbox{EMD-Net}({\bf B}, \mathcal{E}_{\mathcal{T}}),
% \end{equation} 
% where $\mathcal{E}_{\mathcal{T}} \triangleq \{({\bf x}_i,p_i,t_i)\}_{t_i\in \mathcal{T}}$ is the set of events triggered in $\mathcal{T}$ with $t_i$ and ${\bf x}_i$ respectively denoting the timestamp and the pixel location of the $i$-th event, and $p_i\in \{+1,-1\}$ denoting the polarity. EMD-Net is also a {\bf $\mathbf{1}$-to-many} operator and once it has been trained, only latent clear images of fixed timestamps $t_n$ can be predicted. And an interpolation network is required to restore the latent images off the fixed timestamps \cite{lin2020learning}, which increases the complexity and even results in sub-optimal solutions.
% Different from \eqref{eq:deblurNet}, the task of DeMo aims at the {\bf $\mathbf{1}$-to-$\mathbf{\infty}$} restoration of clean and sharp latent images of any timestamp $t$ during the exposure time interval $\mathcal{T}$. It can be realized by learning an implicit neural representation \cite{niemeyer2019,mildenhall2020c,pumarola2020,tretschk2021}, \ie,
% \begin{equation}\label{eq:demo}
%     {\bf I}(t) = \mbox{DeMo}(t; {\bf B}, \mathcal{E}_{\mathcal{T}}), \forall t\in \mathcal{T},
% \end{equation}
% which is an implicit video function (IVF) of time $t$ conditioned by a single blurry image $\bf B$ and event streams $\mathcal{E}_{\mathcal{T}}$. In our setting, learning a DeMo is struggling from two aspects
% \paragraph{Event Noises} Events properly bridge the blurry image $\bf B$ and its latent images $\bf I$, providing a naive model for DeMo,
% \begin{equation}\label{eq:edi}
% \tilde{\bf I}(t) = \tilde{\bf B} - \tilde{\bf E}(t;\mathcal{E}_{\mathcal{T}}),
% \end{equation}
% with $\tilde{\bf B},\tilde{\bf I}$ and $\tilde{\bf E}$ are respectively the logarithms of $\bf B$, $\bf I$ and the event-based double integral (EDI) \cite{pan2019bringing}. 
% However, event noises are enormous both in spatial and temporal domains \cite{inivaiton2020}, which might be accumulated in EDI \cite{wang2020event}, resulting in considerable image degradation \cite{pan2020high} especially in the static background.
% \paragraph{Learning IVF from Blurry Images} The IVF learning is intuitively inspired from the implicit neural representation, where videos can be represented as the function of time and position in the continuous form \cite{niemeyer2019}. However, existing IVF approaches require multi-frame inputs with sharp and clear formation \cite{Bemana2020xfields}. Clearly, learning the IVF from blurry images is more challenging than existing IVF tasks due to the motion ambiguities and texture erasures. 
% Above two challenges are coupled together. On one hand, the high temporal resolution of events provides the intra-frame information that can effectively boost the DeMo performance. On the other hand, the learned DeMo implicitly reflects scene dynamics which can be effectively employed to reduce event noises. Thus, one should fulfill the task of DeMo with attention to both {\it event noise suppression} (ENS) and {\it blurry feature enhancement} (BFE).
%\input{fig/overview}
%\begin{figure}[]
%	\begin{center}
%		\includegraphics[width=0.89\columnwidth,trim={0 2.5cm 0 0},clip]{fig/net_x2}
%	\end{center}
%	\vspace{-0.5em}
%	\caption{Overview of the DeMo-IVF where $f_\gamma$ is a feature embedding network and $\phi_\theta$ is a continuous-time decoding MLP.\vspace{-1.5em}}
%	\label{fig:overview}
%\end{figure}
%\begin{figure}[]
%	\begin{center}
%		\includegraphics[width=.89\columnwidth]{fig/net_x1}	
%	\end{center}
%	\vspace{-.5em}
%	\caption{DFEN (upper block) and its dual attention blocks (DALS, bottom block).\vspace{-1.5em}}
%	\label{fig:dals}
%\end{figure}
%	\begin{subfigure}[t]{0.48\linewidth}
%	\includegraphics[width=0.89\columnwidth,trim={0 2.5cm 0 0},clip]{fig/net_x2}
%	\label{fig:overview}
%\end{subfigure}
%\begin{subfigure}[t]{0.48\linewidth}
%	\includegraphics[width=.89\columnwidth]{fig/net_x1}	
%	\label{fig:dals}
%\end{subfigure}

% \subsection{Implicit Video Function}\label{sec:ivf}/



\noindent\textbf{Relation to EDI~\cite{pan2019bringing}.} Events properly bridge the blurry image $\bf B$ and its latent images $\bf I$, providing a naive model for DeMo,
\begin{equation}\label{eq:edi}
\tilde{\bf I}(t) = \tilde{\bf B} - \tilde{\bf E}(t;\mathcal{E}_{\mathcal{T}}),
\end{equation}
with $\tilde{\bf B},\tilde{\bf I}$ and $\tilde{\bf E}$ are respectively the logarithms of $\bf B$, $\bf I$ and the event-based double integral (EDI) \cite{pan2019bringing}. The IVF in \cref{eq:ivf} and the EDI in \cref{eq:edi} can both tackle the DeMo task by shifting the original deblurring problem to the restoration of the TA component. However, EDI calculates the TA component by accumulating per-pixel events \cite{wang2020event}, thus its performance might be degraded due to the event noise \cite{inivaiton2020} and incorrect estimation of the event threshold \cite{pan2020high}. Compared to EDI, our IVF attempts to learn the TA component by dual feature embedding (described in the next section), which leverages the merits of the blurry image $\bf B$ and events $\mathcal{E}_{\mathcal{T}}$ with the consideration of following issues: (1) suppression of event noise with the guidance of image features; (2) deblurring features extracted from the blurry input $\bf B$ with the enhancement of event features. 
% However, the event noise is severe both in spatial and temporal domains \cite{inivaiton2020}, which may be accumulated in EDI \cite{wang2020event}, resulting in considerable image degradation \cite{pan2020high}. %especially in the static background.

\noindent\textbf{Relation to INR~\cite{niemeyer2019,Bemana2020xfields}.} IVF learning is intuitively inspired by Implicit Neural Representation (INR), where videos can be represented in continuous form as a function of time and location \cite{niemeyer2019}. However, existing INR approaches generally require multi-frame inputs with clear information \cite{Bemana2020xfields}. Thus, learning an IVF from a blurry image is more challenging than existing INR learning tasks due to motion ambiguity and texture erasure. 

% The above two challenges are coupled together. On one hand, the high temporal resolution of events provides the intra-frame information that can effectively boost the performance of DeMo. On the other hand, the learned DeMo implicitly reflects scene dynamics which can be employed to reduce event noise. Thus, one should complete the task of DeMo with attention to both event noise suppression and blurry feature enhancement.


%Thus,  (3) jointly estimating the TA component with the fusion of enhanced event features and deblurred image features. 
% IVF \cref{eq:ivf} and EDI \cref{eq:edi} can tackle the DeMo task by shifting the original deblurring problem to the restoration of the TA components. The difference is that the IVF attempts to learn the TA components by dual feature embedding, which leverages the merits of the blurry image $\bf B$ and the concurrent events $\mathcal{E}_{\mathcal{T}}$ for (1) suppressing event noises with the guidance of image features; (2) deblurring  features extracted from $\bf B$ with the enhancement of event features; (3) jointly estimating the TA components with the fusion of event features and deblurred image features. However, EDI calculates the TA components only by accumulating events in a pixel-wised manner. Thus to some extent, the IVF can be considered as a generalization of the EDI model in the intensity domain (EDI is in the logarithmic domain), but more robust to event noises than EDI since it combines information from the blurry image and events.
\cref{fig:overview_dals} illustrates the proposed network to fulfill the IVF in \cref{eq:ivf}. Accordingly, the overall network architecture contains two modules, \ie, the module of dual feature embedding $f_\gamma$ and the module of continuous-time decoding MLP $\phi_\theta$.

\subsection{Dual Feature Embedding Network}
\label{sec:DFEN}
% As discussed in \cref{sec:ivf}, we are interested in developing a network to take the merits of both event streams and images for feature embedding. Accordingly, we build our Dual Feature Embedding Network (DFEN) to embed those two sources of information in a unified embedding space.
To achieve the mutual compensation of events and frames, we design a Dual Feature Embedding Network, \ie, DFEN, to embed those two sources of information in a unified embedding space.
Our DFEN initializes the input blurry image $\mathbf{B}$ and the event stream $\mathcal{E}_\mathcal{T}$ by a {\color{black}{Shallow Feature Extraction (SFE) module}} using the pixel shuffling~\cite{shi2016} operation with a stride of $2$, and then uses two convolution blocks to transform the features of events and the blurry image into feature maps with $C$ channels, denoted by $\mathbf{B}_{feat}, \mathbf{E}_{feat} \in\mathbb{R}^{C\times \frac{H}{2} \times \frac{W}{2}}$. 
% With the initialized features $\mathbf{B}_{feat}, \mathbf{E}_{feat}$,
We then leverage several Dual Attention blocks to take into account the Latent Structures (DALS) shared with the dual input features $\mathbf{B}_{feat}$ and $\mathbf{E}_{feat}$, as shown in \cref{fig:overview_dals}. Each DALS block is composed of a
{\color{black}{Residual Dense Block (RDB)}} \cite{zhang2018residual} and a Window-based Multi-head Self-Attention (W-MSA) block in a sequential manner, where a Dual Attention Mechanism (DAM) is implemented in DALS for event noise suppression and blurry feature enhancement.

% we use the Window-based Multi-Head Self Attention (W-MSA) layers to exploit the latent structures from two information sources, which finally yields a unified feature embedding for the dual inputs.

% With the initialized features $\mathbf{B}_{feat}, \mathbf{E}_{feat}$, we use the Window-based Multi-Head Self Attention (W-MSA) layers to exploit the latent structures from two information sources, which finally yields a unified feature embedding for the dual inputs.
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{fig/fig_method/dals.jpg}
\caption{Detailed Dual Attention block to take into account the Latent Structures (DALS) shared with the dual input features $\mathbf{B}_{feat}$ and $\mathbf{E}_{feat}$.}
\label{fig:overview_dals}
\end{figure}

\noindent \textbf{Window-based Multi-head Self-Attention (W-MSA).} We follow the basic strategy proposed in \cite{liu2021c} to first partition the features $\mathbf{F}\in\mathbb{R}^{C\times h\times w}$ into $L$ local patches, and then calculate the self-attention by $$\text{W-MSA}(\text{Attn}, V) = \text{Attn} \cdot V$$ with the self-attention weight defined as $\text{Attn}=\text{softmax}(\frac{QK^T}{\sqrt{d_k}})$, where $Q$, $K$ and $V$ are the encoded queries, keys and values, yielded by an MLP for each of them. Different from the case of uni-modal input in \cite{liu2021c}, we further propose the DAM to modify the self-attention weights for mutual compensation of multi-modal signals.

% For a feature map $\mathbf{F}\in\mathbb{R}^{C\times h\times w}$, we follow \cite{liu2021c} to partition the features $\mathbf{F}$ into $L$ local patches, denoted by $\mathbf{F}_{0},\ldots, \mathbf{F}_{L-1} \in \mathbb{R}^{C\times m\times m}$. 
% For each feature patch $\mathbf{F}_i$, we first compute the self-attention weight by $\text{Attn}=\text{softmax}(\frac{QK^T}{\sqrt{d_k}})$, and then generate the self-attention by 
% $
%     \text{W-MSA}(\text{Attn}, V) = \text{Attn} \cdot V,
% $
% where $Q$, $K$ and $V$ are the encoded queries, keys and values, yielded by MLP for each feature.

% \noindent \textbf{Window-based Multi-head Self Attention.} For a feature map $\mathbf{F}\in\mathbb{R}^{C\times h\times w}$, we follow \cite{liu2021c} to partition the features $\mathbf{F}$ into $L$ local patches, denoted by $\mathbf{F}_{0},\ldots, \mathbf{F}_{L-1} \in \mathbb{R}^{C\times m\times m}$. For each feature patch $\mathbf{F}_i$, we compute the attention by
% $
%     \text{W-MSA}(Q, K, V) = \text{softmax}(\frac{QK^T}{\sqrt{d_k}}) V,
% $
% where $Q$, $K$ and $V$ are the encoded queries, keys and values, yielded by MLP for each feature.

% \noindent \textbf{Dual Attention with Latent Structures.} 
% As shown in \cref{fig:overview_dals}, we leverage several Dual Attention blocks to take into account Latent Structures (DALS) shared with the dual input features $\mathbf{B}_{feat}$ and $\mathbf{E}_{feat}$. Each DALS block is composed of a
% {\color{black}{Residual Dense Block (RDB)}} \cite{zhang2018residual} followed by a W-MSA block in a sequential manner. 
\noindent \textbf{Dual Attention Mechanism.} 
In the $i$-th ($1\leq i \leq N$) W-MSA block, two parallel paths are designed to firstly compute the self-attention weights $\text{Attn}_{E}$ and $\text{Attn}_{B}$ for the features of events and images. We then propose a dual attention mechanism to mutually compensate the event features and image features.
Firstly, as the input events usually contain unexpected noise, we use the learned attention weight $\text{Attn}_{B}$ from the blurry features (less noisy) to calibrate the attention weights $\text{Attn}_{E}$ by 
\begin{equation}\label{eq:atten_e0}
    \mbox{Attn}_{E} \leftarrow \mbox{Attn}_{E} + \mbox{Attn}_{B}.
\end{equation}
Once the attention weight $\text{Attn}_{E}$ is calibrated, we compute the event features from $\mathbf{E}_{feat}^{i-1}$ by
\begin{equation}\label{eq:atten_e}
\begin{split}
\bar{\mathbf{E}}_{feat}^{i-1} &= \text{W-MSA}(\mbox{Attn}_E^{i-1},V(\mathbf{E}_{feat}^{i-1})),
% \mbox{Attn}_E^{i-1} \cdot V(\mathbf{E}_{feat}^{i-1}), 
\\
\mathbf{E}_{feat}^i &= \text{MLP}_E^{i-1}(\bar{\mathbf{E}}_{feat}^{i-1}),
\end{split}
\end{equation}
where $V(\cdot)$ is the corresponding value operator. 
Such a design suppresses the incorrectly-estimated attention for the noisy events, leading to the enhancement of event features from the blurry image. %({\bf B2E}).
On the other hand, the image features often suffer from the loss of textures due to the blur degradation, which can be potentially compensated by events.
% extracted from the blurry inputs are often  suffer from blurry textures, which can be further eliminated benefiting from the low latency of events. 
To achieve this end, we compute the image features from both $\mathbf{B}_{feat}^{i-1}$ by
\begin{equation}\label{eq:dual-attn}
\begin{split}
    \bar{\mathbf{B}}_{feat}^{i-1} &=
    \text{W-MSA}(\text{Attn}_B^{i-1},V(\mathbf{B}_{feat}^{i-1})),
    % \text{Attn}_B^{i-1} \cdot V(\mathbf{B}_{feat}^{i-1}), 
    \\
    \mathbf{B}_{feat}^i &=\text{MLP}_B^{i-1}([\bar{\mathbf{B}}_{feat}^{i-1};\bar{\mathbf{E}}_{feat}^{i-1}]),
\end{split}
\end{equation}
where $\bar{\mathbf{E}}_{feat}^{i-1}$ is the weighted event features computed from \cref{eq:atten_e}. The feature concatenation compensates the image features with the texture information from the event features, leading to deblurring effects. %({\bf E2B}).
% the texture ambiguities, leading to deblurring effects from event features ({\bf E2B}).

% Then 
% \begin{equation}
%     \begin{split}
%     \mathbf{B}_{feat}^i &= \text{MLP}_B^{i-1}([\mathbf{B}_{feat}^{i-1};\mathbf{E}_{feat}^{i-1}])\\
%     \mathbf{E}_{feat}^i &= \text{MLP}_E^{i-1}(\mathbf{E}_{feat}^{i-1})
% \end{split},
% \end{equation}

Combining Eqs.~\eqref{eq:atten_e0}, \eqref{eq:atten_e}, and \eqref{eq:dual-attn}, we firstly calibrate the attention weights $\text{Attn}_E$ for events by using the contextual information from the blurry image features to obtain better event features.
 Then, the enhanced event features are concatenated with the initial image features for further refinement. As the partitioning operation splits an image plane into non-overlapped regions, we use the shifting operation for the blocks with even indices to keep the consistency between non-overlapped patches. 
%  In summary, we call this mechanism as Dual Attention with Latent Structures (DALS). 
 Finally, we concatenate the output image features (with the inverse partitioning operation) of all DALS blocks into $\mathbf{F}_{cat} \in \mathbb{R}^{NC\times h\times w}$ as the feature embedding. In our implementation, the number of DALS blocks is set to $20$. 
% Nan: do we need to use ablation study to justify our design?
    
% \paragraph{Event Noise Suppression via Cross-Modality Attention}
% 通过image的attention weight，加权event，去噪声

% \paragraph{Feature Deblurring via Post-Attention Fusion}
% 通过event attention之后的结果，对image的feature（模糊）进行多级融合去模糊
% 这里我说的是前面每个W-MSA的V的融合
With the learned high-dimensional feature embedding, we combine the initial features $\mathbf{B}_{feat}$ extracted from the blurry image with the outputs of all W-MSA blocks {\color{black}{by a Global Feature Fusion (GFF) module}}. Specifically, we use a $1\times 1$ convolution layer to firstly reduce the feature channels from $N\times C$ to $C$ and then use a $k\times k$ convolution layer to generate the deblurred features $\mathbf{F}_{db}$ by
\begin{equation}
    \mathbf{F}_{db} = \mathbf{B}_{feat} + \text{Conv}_{k\times k}(\text{Conv}_{1\times 1}(\mathbf{F}_{cat})).
\end{equation}

\subsection{Continuous-Time Decoding MLP}

\begin{figure}[t]
\centering
\includegraphics[width=0.35\textwidth]{fig/fig_method/MLP.jpg}
\caption{Details of Continuous-time Decoding MLP, which accepts the deblurred feature $\mathbf{F}_{db}$ output by DFEN and the embedding of any specified time $\eta(t)$ to decode the latent sharp image $\mathbf{I}(t)$.
} 
\label{fig:continuous-time decoding}
\end{figure}
As our feature embedding network encodes the temporal information, we propose to query the sharp image at an arbitrary timestamp in the range of the imaging exposure period. Without loss of generality, we normalize the exposure time interval into units and query the normalized timestamp $t \in [0,1]$. For the query time $t$, we encode it into a high-dimensional vector $\eta(t) \in \mathbb{R}^{2L}$ ($L=8$ in our experiment) following the Fourier encoding scheme used in \cite{benbarka2021},
\begin{equation}\small 
    \eta(t) = 
    \begin{pmatrix}
    \cos(2^0\pi t), \sin(2^0\pi t), \ldots, \cos(2^{L-1}\pi t), \sin(2^{L-1}\pi t)
    \end{pmatrix}.
\end{equation}
After decoding the query image at timestamp $t$, we apply a pixel-shuffle layer and convolution layers to upsample the deblurred feature $\mathbf{F}_{db}$ into $\mathbf{F}_{db}^{\uparrow} \in \mathbb{R}^{32\times H\times W}$ to keep the original image resolution. Following that, we concatenate the time embedding $\eta(t)$ in each pixel to yield a time-specific feature map and then use an MLP with four $256$-D hidden linear layers to finally decode the sharp latent frame at time instance $t$, denoted by $\mathbf{I}(t)$. Unlike the previous approaches that only produce the latent images at fixed timestamps, our time-continuous decoding module is able to restore the sharp images at any given time instances $t$.

 Given a single blurry image $\mathbf{B}$ and its concurrent event stream $\mathcal{E}_\mathcal{T}$, one can first use the DFEN module for feature embedding and then get the deblurred features $f_\gamma(\mathbf{B},\mathcal{E}_\mathcal{T})=\mathbf{F}_{dblr}$, which are time constant. In the continuous-time decoding MLP, we only need to change the value of time $t$ to restore the TA component $\phi_\theta$ of the latent image $\mathbf{I}(t)$, and then add it to the blurry image $\mathbf{B}$ to reconstruct $\mathbf{I}(t)$. 
 % Thus, once the feature embedding is learned, the inference of $\mathbf{I}(t)$ by DeMo-IVF is computationally efficient. \textcolor{red}{(ZX: should we add a computational complexity exp to support this claim?)}

%\input{fig/gopro}
% In our setting, $L$ is equal to $3$ and $\left [ P_1, P_2, P_3 \right ]$ is equal to $\left [ 3000, 5000, 7000\right ]$.
% and that the events accumulated over a short period of time exactly reflect the appearances of the image edges at the corresponding moments.

% supervision by finite frames (GT)

% flow consistency

% intensity consistency
\input{tab/tab_gopro_hqf_7.tex}

\subsection{Motion and Texture Guided Supervisions}
% We learn the implicit video function with sparsely sampled sharp images captured in $K$ timestamps $T_K = \{t_i\}_{i=1}^{K}$ in the exposure interval.  Let $\mathcal{\hat{I}} = (\mathbf{\hat{I}}_{t_1}, \ldots \mathbf{\hat{I}}_{t_K})$ be the ground-truth images. It is straightforward to use the $\ell_1$ loss to optimize our DFEN $f_\gamma$ and decoding MLP $\phi_\theta$, \ie,
% \begin{equation}\label{eq:loss-im}
%     \mathcal{L}_{im} = \frac{1}{K} \sum_{i=1}^K \|{\bf I}(t_i) - \mathbf{\hat{I}}_{t_i}\|_1.
% \end{equation}

% For a single blurry image $\mathbf{B}$ and the corresponding event stream $\mathcal{E_T}$, there exists $K$ timestamps $T_K = \{t_i\}_{i=1}^{K}$ and ground-truth images $\mathcal{\hat{I}} = (\mathbf{\hat{I}}_{t_1}, \ldots \mathbf{\hat{I}}_{t_K})$ in the exposure interval.
%pairs of timestamps and ground-truth images $\left\{ \left( t_k, \mathbf{\hat{I}}(t_k) \right) | 1 \le k \le K, t_k \in \mathcal{T} \right\}$. 

We learn the implicit video function with sampled sharp images captured in $K$ timestamps $T_K = \{t_i\}_{i=1}^{K}$ in the exposure interval. Let $\mathcal{\hat{I}} = (\mathbf{\hat{I}}({t_1}), \ldots \mathbf{\hat{I}}({t_K}))$ be the ground-truth images.
It is straightforward to use the $\ell_1$ loss to optimize our DFEN $f_\gamma$ and decoding MLP $\phi_\theta$, 
\begin{equation}\label{eq:loss-im}
    \mathcal{L}_{im} = \frac{1}{K} \sum_{k=1}^K \|{\bf I}(t_i) - \mathbf{\hat{I}}({t_i})\|_1.
\end{equation}
It can be foreseen that as $K$ increases, \ie, more data with ground-truth images of different timestamps are used for supervision, the trained model will achieve the continuous-time video extraction task better.
However, due to practical constraints such as limited camera frame rates, for one single blurry image, we can only acquire a few pairs of timestamps and sharp images as the supervision signals.  
Restricted by the sparse sampling, only using \cref{eq:loss-im} over all the supervision samples is not enough for our goal of continuously decoding sharp images at any given time $t$. And in our experiments, we found that such a treatment will lead to a bias in the sparsely sampled timestamps. 
% Therefore, the continuity of the time should be considered in the training phase of the network. 

% \vspace{-1em}
% \paragraph{Flow Consistency} 
% We address the bias issue caused by the sparse samples using event-based optical flow. 
% Ideally, if an optical flow is obtained from the already-sampled time $t_k$ to any time $t = t_k + \delta$, it is feasible to warp the sharp image $\mathbf{\hat{I}}_{t_k}$ to a sharp image at time $t$ as the  ground-truth for learning. 
% However, due to the lack of optical flow between any timestamp, we alternatively use an off-the-shelf method EV-Flow~\cite{zhu2018ev} to yield the pseudo flow maps $\text{Flow}_{t_i\to t}=\text{EV-Flow}(\mathcal{E}_{t_i\to t})$, with $\mathcal{E}_{t_i\to t}$ denoting events triggered during $[t_i, t]$. %\textcolor{red}{Nan: please add the detail of how to sample time $t$ for flow consistency.}
\noindent{\bf Motion-Guided Supervision.}
To address this problem, we introduce motion-guided supervision that allows the model to exploit motion continuity to achieve continuous-time video extraction. The key idea is utilizing the motion information encoded in events to bridge the inter-frame connection between the latent sharp images.
Ideally, if an optical flow $\text{Flow}_{t_i \to t_i + \delta}$ is obtained from the already-sampled time $t_i$ to any time $t = t_i + \delta$, it is feasible to warp the sharp image $\mathbf{\hat{I}}(t_i)$ to a sharp image at time $t$,
\begin{equation}
    \mathbf{\hat{I}}(t_i + \delta) = \text{Warp} \left ( \mathbf{\hat{I}}(t_i), \text{Flow}_{t_i \to t_i + \delta} \right ) ,
\end{equation}
By establishing the above motion connections, the data outside of sampling distribution can be obtained as the extra supervised signals.
However, due to the lack of optical flow between any timestamp, we alternatively use an off-the-shelf method EV-Flow~\cite{zhu2018ev} to yield the pseudo flow maps $\text{Flow}_{t_i\to t}=\text{EV-Flow}(\mathcal{E}_{t_i\to t})$, with $\mathcal{E}_{t_i\to t}$ denoting events triggered during $[t_i, t]$. %\textcolor{red}{Nan: please add the detail of how to sample time $t$ for flow consistency.}

In detail, we randomly sample $M$ timestamps $\{t_j^{\prime} \}_{j=1}^{M}$ (For clarity, we refer to the timestamps in $T_k$ where real ground truth can be obtained as the Referenced timestamps and the timestamps outside of it as the Non-referenced timestamps.).
For each Non-referenced timestamp $t_j^{\prime}$, $N$ nearest Referenced timestamp $ \{t_{j, k} \}_{k=1}^{N} (N \leq K)$ are obtained from $T_K$ (\ie, $t_{j, k} \in T_K$).
We use events to compute the optical flow from $t_{j,k}$ to $t_j^{\prime}$ and warp the image $\mathbf{\hat{I}}({t_{j,k}})$ to $\mathbf{\hat{I}}^k({t_j^\prime})$, and then compute the motion loss to calibrate the image prediction without references,
\begin{equation}  
    \mathcal{L}_{motion} = \frac{1}{M \times N} \sum_{j=1}^M \sum_{k=1}^N \left\|{\bf I}(t_j^\prime) - \hat{{\bf I}}^k({t_j^\prime})\right\|_1.
\end{equation}
where $\hat{{\bf I}}^k({t_j^\prime}) = \text{Warp}(\mathbf{\hat{I}}({t_{j, k}}), \text{Flow}_{t_{j, k}\to t_j^\prime})$.
Jointly supervising ${\bf I}(t_j^\prime)$ by multiple $\{ \hat{{\bf I}}^k({t_j^\prime}) \}_{k=1}^{N}$ warped from $N$ ground-truth images at different Referenced timestamps can help to alleviate distortions caused by mispredicted optical flow. 

With the aid of motion loss, our network learns to utilize temporal consistency to restore a more continuous and smooth video. Nevertheless, we found that slight blurring and artifacts are still present in the estimates. This is mainly caused by two factors. 
First, the optical flow used in motion loss is predicted from the event stream, and exists some errors, especially in the regions with meticulous textures and small motions. These errors will further affect the reconstruction of our network in the corresponding areas.
% Second, we convert the raw event stream $\mathcal{E}$ into event images before input to the network. 
Second, before the raw event stream $\mathcal{E}$ is input to the network, it will be evenly divided into multiple intervals according to time and then the events in each interval are accumulated into the event images. In this process, the temporal information within the interval will be lost due to accumulation, which is conducive to image restoration at these moments. As the cumulative number of events increases, the loss of information becomes more serious. When too many events are generated due to fast movement, the converted event images will be blurry with thick accumulated edges and may even suffer from motion overwriting problems such that the network has difficulty in extracting detailed textures of the scene. 
% \cref{fig:EdgeRefine-1} show how these two factors affect the reconstruction.
% \subsection{Event-based Edge Refinement}
\input{fig/fig_reds_hqf.tex}

\noindent \textbf{Texture-Guided Supervision.} 
% The IVF model trained with the above method is able to predict the continuous illumination change for each pixel from the blurry image with the aid of events, thus restoring the latent sharp images at arbitrarily specified timestamps. 
% Nevertheless, we found that slight blurring and artifacts are still present in the estimates. This is mainly caused by two factors. 
% First, the deep neural network is biased towards learning lower frequency functions ~\cite{mildenhall2020c, rahaman2019spectral} and thus tend to predict continuous illumination that vary smoothly over time. The temporal smoothing effect will lead to smoother spatial variation and eventually result in the blurring effect on the edges. This phenomenon is more severe for the reconstruction of non-key timestamps because the corresponding supervised images obtained by interpolation are relatively degraded and blurred. 
% Second, as said in \cref{sec:}, we convert the raw event stream $E$ into event images before input to the network. However, when too many events are generated due to fast movement, the converted event images will be blurry with thick accumulated edges and may even suffer from motion overwriting problems such that the network has difficulty in extracting detailed textures of the scene to reconstruct sharp edges. 
% \cref{fig:EdgeRefine-1} show how these two factors affect the reconstruction.
% as shown in \cref{fig:EdgeRefine-2}, when predicting latent sharp images at multiple moments from the same blurred image, the image reconstructed with more events near the corresponding moment will be relatively more blurred.
% It is difficult to completely eliminate the influence of these two factors in the above frameworks.
% Nevertheless, we observe that they mainly have an impact on the reconstruction of the edge regions that are exactly located where (and when) events occur \cite{pan2019bringing}. 
To alleviate the impact of these two factors, we further propose texture-guided refinement to compensate for the loss of intermediate information and to recover better textures and details.
In detail, we introduce the Event-based Edge Refinement ($\operatorname{EER}$) module to refine the initial deblurring results ${\mathbf I}(t)$ with the guidance of the events, \ie, 
\begin{equation}
    {\mathbf I}_{\mathrm{refine}}(t) = \operatorname{EER} \left ( {\mathbf I}(t),  \mathcal{E}_t \right ),
\end{equation}
where ${\mathbf I}_{\mathrm{refine}}(t)$ indicates the refined image result and $\mathcal{E}_t$ indicates the events corresponding to timestamp $t$.
% 定义local event
Specifically, supposing $\mathcal{E}_{\ge t}^{P}$ ($\mathcal{E}_{\le t}^{P}$) the set of $P$ events with timestamps that are nearest to and greater (less) than $t$, $\mathcal{E}_t$ is defined as follow, 
\begin{equation}
    \mathcal{E}_t = \left \{ \mathcal{E}_{\ge t}^{P_1}, \mathcal{E}_{\le t}^{P_1}, ..., \mathcal{E}_{\ge t}^{P_L},  \mathcal{E}_{\le t}^{P_L}  \right \},
\end{equation}
where $2L$ sets with different numbers of events are grouped together to provide rich and accurate information with the consideration that the event rates vary for different samples and also vary for different image regions of the same sample.
The $\operatorname{EER}$ module extracts the edge structures from the events to refine the initial deblurring results. We implement it as the neural network and learn the task from data.
% Unlike the training process of the IVF model, the data on the non-key-timestamps is not used here, in order to avoid the introduction of edge blur by interpolation.

% 与已有方法进行比较
Our EER module shares the same key idea as the DEF module proposed in LEMD\cite{jiang2020learning}, which enhances the reconstruction with the aid of sharp edge prior extracted from events. 
DEF gets the edge guidance map by sampling events between two latent sharp images, while EER directly uses events near the enhanced target to provide edge priors, which is easier to implement and avoids sampling errors.
Moreover, DEF is incorporated into the main network to provide edge priors for the reconstruction of each predefined timestamp, which is not feasible for IVF because the target of the reconstruction is determined by the additional input $t$.
Therefore, the EER is designed as a stand-alone module that refines the initial estimates, which is more compatible with the IVF model and can be cascaded to any other event-based deblurring method for edge refinement.

\noindent \textbf{Training strategy.}
The whole training process is composed of two phases. 
In the first phase, we optimize our IVF model using $\mathcal{L}_{im}$ and $\mathcal{L}_{motion}$, 
% Stage 1: 
% The final loss function is 
% % \input{tab/sota.tex}
\begin{equation}\label{eq:allloss}
% \small 
    \mathcal{L}_{total} =\lambda_1 \mathcal{L}_{im}  + \lambda_2 \mathcal{L}_{motion}.
\end{equation}
with $\lambda_1$ and $\lambda_2$ being the balancing parameters.
The model trained in the first stage is able to predict the continuous illumination change for each pixel from the blurry image with events, thus restoring the latent sharp images at arbitrarily specified timestamps. 
In the second phase, we fix the parameters of the well-optimized IVF model and use it to estimate the initial deblurring results in the Reference timestamps $t_i$, which are then fed into the $\operatorname{EER}$ module along with the corresponding events $\mathcal{E}_{t_i}$.
\begin{equation}
    {\mathbf I}_{\mathrm{refine}}(t_i) = \operatorname{EER} \left ( \mbox{DeMo}(t_i; {\bf B}, \mathcal{E}_{\mathcal{T}}),  \mathcal{E}_{t_i} \right ),
\end{equation}
The $\ell_1$ loss between the refined results ${\mathbf I}_{\mathrm{refine}}(t_i)$ and the ground truth images $\mathbf{\hat{I}}({t_i})$ is used to optimize the $\operatorname{EER}$ module,
\begin{equation}
    \mathcal{L}_{refine} = \frac{1}{K} \sum_{i=1}^K \|{\mathbf I}_{\mathrm{refine}}(t_i) - \mathbf{\hat{I}}({t_i})\|_1,
\end{equation}
After two stages of training, IVF and EER together achieve extracting continuous-time sharp video with delicate details from the blurry image and events.

\input{tab/tab_reds_31.tex}
\input{fig/fig_reds_31.tex}
\input{fig/fig_rbe.tex}




==> sec/4_results.tex <==
\section{Experiments and Analysis}
% \vspace{-1cm}
% \input{fig/fig2.tex}

\subsection{Experimental Settings}
\noindent {\bf Datasets.} 
% =======================
% Training Set
The task of DeMo-IVF is fulfilled via learning an implicit video function supervised by synthetic datasets, \ie, {REDS} \cite{Nah_2019_CVPR_Workshops_REDS} and {HQF} \cite{stoffregen2020reducing}, where the Ground Truth (GT) latent sharp images are available. 
% How to process REDS dataset
% Specifically, the {REDS} dataset is composed of simulated blurry images and events which are synthesized as \cite{xu2021motion}. 
Specifically, the original REDS dataset contains 270 videos captured at 120 fps and each video contains 500 sharp and clear images at resolutions of $720 \times 1280$. We convert all videos to grayscale image sequences and downsample them to $180 \times 320$. After that, we use the frame interpolation algorithm ~\cite{huang2022real} to increase the frame rate. Based on the interpolated image sequences, we generate event streams with the ESIM\cite{rebecq2018esim} simulator and synthesize blurry images by merging subsequent frames. To facilitate algorithm comparison on continuous-time restoration (\cref{comparison}), we use 31 sharp images (before interpolation) to synthesize one blurry image. We follow \cite{Nah_2019_CVPR_Workshops_REDS} to split these videos into the train and test subsets with 240 and 30 videos.
% How to process HQF dataset
The HQF dataset contains real events and high-quality sharp images captured simultaneously by a DAVIS240 camera where the images are minimally blurred. 
We use the same approach as the REDS dataset (interpolation and merging) to simulate motion blur. Due to its relatively low frame rate, only 7 sharp images are merged into one blurry image for HQF. % To simulate motion blur, we first increase the frame rate by interpolating 7 images between consecutive frames using RIFE \cite{rife_huang2020rife}, and then generate 1 blurry image by averaging 49 neighboring sharp frames.

% =======================
% Testing Set
The trained model is evaluated over three different datasets, \ie, REDS\cite{Nah_2019_CVPR_Workshops_REDS}, {HQF}\cite{stoffregen2020reducing}, and {RBE} \cite{xu2021motion}.
We carry out the quantitative and qualitative comparisons over the REDS and HQF datasets since they both contain paired ground-truth images.
% The REDS and HQF datasets both have paired Ground Truth (GT) and blurry inputs, thus we carry out the quantitative experiments over REDS and HQF. 
The RBE dataset \cite{xu2021motion} employs a DAVIS346 camera to collect real-world blurry videos and the corresponding event streams (without GT), which is used to evaluate the performance of DeMo-IVF in real-world scenarios.

% is composed of real-world events and motion blurs (without GT) captured with the DAVIS346, thus we exploit it as the qualitative benchmark for latent sharp image restoration of arbitrary timestamp.
% where motion blurs are synthesized for the first two datasets and the RBE dataset is a real-world scenario with real events and real motion blurs. 
% Thus, we carr a{\bf REDS} is synthetic dataset, To achieve this end, we build  where events are simulated by ESIM \cite{}

% \input{fig/fig_gopro_hqf}

\noindent {\bf Training Details.}
Our network is implemented using Pytorch and trained on two NVIDIA GeForce RTX 3090 GPUs.
% with batch size 8 by default. 
The training process is composed of two phases. In each phase, we utilize a batch size of 8 and employ the Adam optimizer \cite{kingma2014adam} with momentum and momentum2 as 0.9 and 0.999.
% The learning rate starts at $3 \times 10^{-4}$ and decays from $25$th to $100$th epoch to $1\times 10^{-5}$,  
And we randomly crop the images to $128 \times 128$ patches and apply random horizontal flipping to them for data augmentation.
% The training dataset is augmented by randomly flipping the input images and cropping them into $128 \times 128$ patches.
During the first phase, the DeMo-IVF network is trained for 400 epochs where the learning rate is $1 \times 10^{-4}$ in the first 50 epochs, linearly decays to $1\times 10^{-5}$ until the $200$-th epoch, and remains unchanged to the end. We set the weighting factors $\lambda_1=1$ and $\lambda_2=0$ in the initial $300$ epochs to stabilize the reconstruction quality of the latent frames at reference timestamps and then modify them to $\lambda_1=0.2$ and $\lambda_2=1$ for the rest 100 epochs to supervise the restoration at arbitrary time instances. For the motion loss $\mathcal{L}_{motion}$, we set the parameters $M=3$ and $N=2$ and employ the optical flow predicted by the EV-Flow network \cite{zhu2018ev} which is pre-trained on the MVSEC dataset~\cite{zhu2018ev} and then fine-tuned with our network in the training stage.
In the second phase, the EER model is trained individually for 200 epochs with the learning rate initialized as $1 \times 10^{-4}$ and decayed by 0.8 every 50 epochs.
% The EV-Flow network \cite{zhu2018ev} is employed for the flow loss $\mathcal{L}_{flow}$ is pretrained on the MVSEC dataset~\cite{zhu2018ev} and fine-tuned with our network in the training stage. 
All input blurry images and the concurrent events are temporally and spatially aligned  before feeding into the network. For an event stream, we first divide it into $6$ segments with equal time intervals and then convert each segment into the accumulated event frame and time surface \cite{zhu2018ev} as the input. 
% Our network is implemented using Pytorch on two NVIDIA Geforce RTX 3090 GPUs.  Adam optimizer is used. .The weighting factors $ \lambda_1 $ and $ \lambda_2 $ are set to 1, 0.5. The number of clear image for supervise is $K=7$. The optical flow module is pretrained on the MVSEC datasets, where the reference ground-truth optical flow is provided.
%\input{fig/gopro_w-o_flow}

% \input{fig/ivf_video}
% \begin{figure}[!th]
%     \centering
%     \includegraphics[width=1.0\linewidth]{fig/tmp_ivf_video.png}
%     \caption{Qualitative comparisons of continuous-time restoration, where $109$ latent images are restored from one single blurry image on the {\it cube} data of the RBE dataset. The first row shows the dynamic video as an animation ({\color{blue}better viewed in Acrobat Reader}), the second and third rows show close-ups of the foreground {\it cube} and the background wall at different timestamps.\vspace{-1.5em}}
%     \label{fig:ivf_infty}
% \end{figure}

\subsection{Single Frame and Sequence Restoration}
\label{comparison}
% 比较了哪些算法
We compare DeMo-IVF with the state-of-the-art frame-based approachs including LEVS\cite{jin2018learning}, Motion-ETR\cite{zhang2021exposure} and event-based methods including EDI\cite{pan2019bringing}, eSL-Net\cite{wang2020event}, LEDVDI\cite{lin2020learning}, RED-Net\cite{xu2021motion} and E-CIR\cite{song2022cir}. LEVS, LEDVDI, and RED-Net can convert one blurry image into a sharp image sequence of length 7, while Motion-ETR, EDI, eSL-Net and E-CIR can recover latent sharp images at arbitrary times as our method.
% Existing motion deblurring approaches mainly focus on converting one blurry image into a single latent image or a video sequence, while our proposed DeMo-IVF aims to recover latent sharp images at arbitrary time instances. Thus, we conduct experiments on both setting.

% \noindent {\bf }
We first evaluate the performance of all methods on the REDS and HQF datasets for conventional motion deblurring tasks of single image reconstruction, \ie, recovering the middle image and video sequence reconstruction with 7 sharp images. 
For the processed REDS dataset, one blurry image corresponds to 31 sharp images, and only 7 images located in specific positions are used for evaluation in this experiment.
The quantitative results are presented in \cref{tab:sota}. As we can see, on the REDS dataset, the proposed method outperforms other methods in terms of both PSNR (up to 1.68 dB improvement) and SSIM (up to 0.0376 improvements). These improvements stem from using the dual attention mechanism(DAM), which allows for a mutual enhancement between the events and the blurry image.
% On the other hand, we also validate the superior performance of DeMo-IVF with real-world events on the HQF dataset. 
On the HQF dataset, our method still performs the best, which also validates the effectiveness of DAM in handling real-world events.

%Note that the inconsistency between the synthesized and real-world events brings a gap to real-world scenarios for most learning based algorithms, including DeMo-IVF-$7$.  Comparing to the methods trained with real events, \ie, RED-Net and LEDVDI,  our proposed DeMo-IVF-$7$ still exhibits better performance in terms of both quantitative and qualitative results (as shown in Fig.~\ref{fig:indoor}), which validates the generalization of our proposed network.
% Thus, the performance drop is considerable for both IVF-$7$ and eSL-Net which only see synthetic events.
% while RED-Net and LEDVDI are trained with real events to reduce the gap to real scenes.
% For the methods trained only with synthetic events, both IVF-$7$ and eSL-Net exhibit a considerable decrease on PSNR since they never see real events.
% It is shown that IVF-$7$ can still achieve the best performance in terms of both PSNR and SSIM. 
% event-based approaches exhibit overwhelming performance deterioration due to the data inconsistency, especially for learning based approaches trained only with synthetic events, \eg, eSL-Net. 
% Since the HQF dataset is built with real events and simulated motion blurs, most algorithms exhibit a large gap between REDS and HQF, for instance, eSL-Net. Although our method is only trained with synthetic events on the REDS dataset without seeing any real events, it still performs well on HQF and exceeds the performance of state-of-the-art methods. Note that the RED-Net and LEDVDI are all trained with real events and adapt to the real scenes, which validates the generalization of our proposed IVF. 

Correspondingly, we demonstrate a qualitative comparison in \cref{fig:reds_hqf_7}, where we select two exemplar restorations respectively from the REDS and HQF datasets. Due to the inherent ambiguities of temporal ordering and lost spatial textures in a blurry image, LEVS and Motion-ETR fail to recover the latent sharp images without the aid of events. The EDI reconstruction is also blurry, possibly caused by the use of total variation as an image quality prior and the assumption of constant triggering thresholds. The output of eSL-Net contains some areas that are too bright or too dark. LEDVDI, RED-Net and E-CIR restore relatively sharp images, but some noticeable noise artifacts remain. Our method achieves the best visual performance and gives sharp edges, smooth surfaces, and clear textures.
% For event-based deblurring methods, the competitors suffer from artifacts and struggle for recovering the clear textures of tiny targets, while our proposed DeMo-IVF achieves the best visual performance among all state-of-the-art methods and gives sharp edges, smooth surfaces, and clear textures.
% Without the help of events, LEVS fails to recover the latent sharp image. For event-based deblurring methods, the competitors suffer from artifacts and give less clear outputs than DeMo-IVF.
%For the task of $1$-to-$\infty$ restoration, the DeMo-IVF is further trained with the overall loss defined in \cref{eq:allloss}, where the optical flow from an arbitrary time $t$ to the reference time $t_i$ is required. 
%We call the resulted model as {\bf DeMo-IVF-$\infty$} as it can query latent images of any time. 
%\cref{tab:sota} gives the quantitative results on both REDS and HQF datasets, where we only evaluate reconstructions at the reference time when GT is available. Qualitative results of the non-reference time reconstructions are shown in Fig.~\ref{fig:infty_seven}. Compared to DeMo-IVF-$7$, DeMo-IVF-$\infty$ improves the visual quality of the non-reference time reconstructions but at the slight sacrifice of performance at the reference time. Despite this setback, DeMo-IVF-$\infty$ still achieves superior performance compared to the state-of-the-art methods.


\subsection{Continuous-time Restoration}
To further explore the ability of DeMo-IVF to recover latent sharp images at arbitrary times, we conduct experiments on reconstructing all 31 frames on the REDS dataset. For Motion-ETR, EDI, eSL-Net, E-CIR and DeMo-IVF, these tasks can be done independently. For LEVS, LEDVDI, and RED-Net, only 7 sharp frames can be restored from one blurry frame, and hence that we insert 4 images between each adjacent deblurred pair with an additional video frame interpolation method \cite{tulyakov2021time} to achieve continuous-time restoration. (7 deblurred images plus $6 \times 4$ interpolated images equals exactly 31 images.)
The quantitative results are presented in \cref{tab:reds_31}. For the methods that perform interpolation after deblurring, LEDVDI and RED-Net have a large performance drop compared to reconstructing only 7 frames, probably because the two-stage method tends to propagate deblurring errors to the interpolation stage and the accumulated errors eventually lead to the performance drop. The results of LEVS do not change much, probably because the recovered images are too blurry and the effect of the interpolation is attenuated. Performance degradation also occurs in the one-stage methods, especially in the learning-based methods. This may be because most learning-based approaches require the representation of events in the form of frames, which is usually achieved by accumulating events over a small period of time, and information lost in the process affects high frame-rate image recovery. To alleviate this problem, our approach chooses the representation of the time surface combined with cumulative events, but it still cannot completely avoid the loss of information. However, in general, our method still has the best performance compared to the one- and two-stage methods. As shown in \cref{fig:reds_31}, the sharp images reconstructed by our method own finer texture and detail, while the image sequence is more consistent and smoother.
% RBE数据集上的结果

To further demonstrate the generalizability of DeMo-IVF on real datasets, we also perform the continuous-time video reconstruction over the RBE dataset with real events and real blurry images. Without ground truth, only the qualitative evaluation can be made and the comparison result are demonstrated in \cref{fig:rbe}. We see that our model is less affected by noise and shows an apparent improvement in perceptual quality.
% For the task of continuous-time restoration, we evaluate the performance of DeMo-IVF over the RBE dataset, which contains real-world motion blurs and events (without GT). We employ the frame-based deblurring method LEVS and the event-based methods eSL-Net and RED-Net for qualitative comparisons. 
% As shown in \cref{fig:ivf_infty}, it is evident that our proposed DeMo-IVF restores the best visual results with fewer artifacts on the foreground {\it cube} surface and better consistency on the background wall. 
% Qualitative comparisons are shown in \cref{fig:ivf_infty} and apparently our proposed DeMo-IVF-$\infty$ has the best visual quality, with fewer artifacts on the foreground {\it cube} surface and more consistencies on the background wall. More visual results are shown in \cref{fig:1}.
% For the task of $1$-to-$\infty$ restoration, we exploit the DeMo-IVF  to query the latent image $\mathbf{I}(t)$ from blurry images in the RBE dataset \cite{xu2021motion} which contains real-world events and motion blurs (without GT). Existing methods can only restore latent images at the reference time $t_i$. Thus, an additional Video Frame Interpolation (VFI) method \cite{bao2019depth} is required to achieve $1$-to-$\infty$ restorations. Qualitative results are shown in \cref{fig:ivf_infty} and apparently our proposed DeMo-IVF-$\infty$ has the best visual quality, with fewer artifacts on the foreground {\it cube} surface and more consistencies on the background wall. More visual results are shown in \cref{fig:1}.

%  We evaluate the performance of reconstructing 7 clear frames or single frame from one blurred image adopted by most current blur-to-video methods.  We trained our network on the synthetic dataset GOPRO. \Table{gopro_and_hqf} shows the results that our method outperforms other methods on REDS in terms of average PSNR (up to 5 dB improvement) and SSIM scores (up to 0.11 improvement). 
% The LEVS method can't obtain the sharp results due to the motion ambiguity and time ambiguity. In contrast, the event-based deblurring method can remove blur with the aid of events. The EDI-based model is very dependent on the estimation of c and the key frame reconstructed at start. In addition, when recovering sharp frames at other moment from the key frame, the more interval events, the worse effect of recovering. The eSL-Net is also trained only on the synthetic dataset REDS, but it ... 
% This suggests that by using the mutual enhancement between event and blur image our method can alleviate the influence of noise and remove blur more effectively.
%% 这里放几张gopro上7帧的对比图

% \paragraph{Results of training with optical flow}
% From \Table{gopro_and_hqf}, we can see that after adding optical flow supervision to the training, the performance on deblurring to 7 frames or one frame will degrade slightly. This is because when training with optical flow, the network needs to learn deblurring and reconstructing clear images at any time, not just 7 images in a fixed position. However, this performance degradation is worth it, because after doing so, we can reconstruct continuous clear images at any time. In fact, we compare the 100 frames reconstructing qualitative results of training with flow and without flow.
% %% 下面放使用光流训练和不使用光流训练的结果差异
% It can be seen that the network trained without optical flow can only reconstruct clear images on the fixed position where ground truth image are provided, for other moments, the reconstructed image has obvious blur artifacts. In contrast, the network trained with optical flow can reconstruct clear image at any time and maintain time continuity.

% \paragraph{Qualitative Results}
% 图放在这里
% {\color{red}Because the existing datasets both have only 7 frames of ground truth, we can't compute the quantitative results of reconstructing super-high frame rate video from one blurry image. So we compare the qualitative result on the RBE datasets with real events and real blur images. For the methods that can only reconstruct 7 frames, we use the frame interpolation method \cite{DAIN} to obtain high-frame rate video. 
% }
% 首先是我们deblur的效果更好（7帧）
% For the results of reconstructing 7 frames by deblurring. we achieve better results than other methods, which is the same as previous results on REDS and HQF. This further illustrates the generalization ability of our model to deal with real blur and real events.
% 然后是对于插入的帧
% For the intermediate frames between these 7 frames, our method can also get a good reconstructing results. In contrast, the results obtained based on frame interpolation have obvious deformation and flickering without using the information of the blur image and event stream, 




\input{tab/tab_ablation.tex}
\input{tab/tab_ablation_flow_er.tex}
\input{tab/tab_noise.tex}

\input{fig/fig_noise}
\input{fig/fig_flow_er.tex}
% \input{fig/fig_flow.tex}

\subsection{Ablation Study}

In this section, we present ablation studies to analyze the design choices of our method. We first demonstrate the performance contribution of each module in the network architecture (\cref{tab:ablation}). Then, we further validate the effectiveness of DAM with additional noise experiments (\cref{tab:noise}, \cref{fig:noise}). Finally, we analyze the role of each step in the training strategy (\cref{tab:reds_flow_er}, \cref{fig:ablation_flow_er}). 

\noindent\textbf{Network Architecture} 
% The proposed method learns the scene dynamics as the IVF from a single blurry image and the concurrent event, which enables the latent image restoration of arbitrary timestamps. It has been shown that the proposed IVF performs favorably against state-of-the-art methods. 
The proposed network architecture is composed of a dual feature embedding network, \ie, DFEN, where the dual feature path and the DAM are designed, an continuous-time decoder MLP and an EER module.
The ablation studies are conducted on the REDS dataset, where the sequence restoration task is considered and 6 different experiments are implemented to analyze the effectiveness of each component, as shown in \cref{tab:ablation}.
% \noindent \textbf{DFEN.}
% First, we build a baseline network with a single feature path (Ex. 1) that directly receives the concatenated blurry image and its event frames. Compared to the models with a dual feature path, the concatenation of two information sources can be considered as a pre-fusion process and thus performs better than the model with only a dual feature path (Ex. 2) and the one without the dual attention mechanism between W-MSA blocks (Ex. 3). As long as the dual attentions are utilized, DFEN outperforms the single path model by a large margin (0.702 dB on REDS and 1.033dB on HQF compared to Ex. 1), which proves the effectiveness of the mutual compensation of the dual features in DFEN.
%Comparing to our proposed multi-stage fusion mechanism, another approach is directly concatenate both the blurry image with event frames as \cite{xu2021motion}. Thus 
% We build two networks with a single path (w/o W-MSA respectively corresponding to Ex. 1 and 2) which directly accept concatenated blurry image and event frame. 
% Compared to dual path approaches (Ex. 3-7), the concatenation of two sources can be considered as a pre-fusion process and thus performs better than Ex. 3 and 4 without dual attentions between W-MSA blocks. As long as the utilization of dual attentions (E2B and B2E, \ie, Ex. 5-8), DFEN outperforms the single path approaches with a large margin (up to 0.702 dB in PSNR compared with Ex. 2), which proves the effectiveness of DFEN.
% \noindent\textbf{W-MSA.}
% The importance of the W-MSA can be validated by comparing Ex. 2 and 3. For the dual path approach, the utilization of W-MSA directly boosts the performance on both REDS and HQF datasets, showing the benefits of self-attention in extracting signal information.
% The utilization of W-MSA (\ie, transformer) slightly reduces performance in single path approach (comparing Ex. 1, 2) and boost performance in dual path approach(Ex. 3, 4).
% The importance of the transformer can be validated by comparing Ex. 2 and 1 (or Ex. 4 and 3). 
% For single or dual path approaches, the utilization of W-MSA can both boost the performance.
% The dual attention mechanism is designed to take the complementary merits of frames and events, where a bidirectional enhancement process is implemented to suppress the noise in event features and simultaneously deblur image features. The comparison of Ex. 3 and Ex. 4 in Tab.~\ref{tab:ablation} shows the importance of DAM in our DFEN in terms of motion deblurring. In DeMo-IVF, the MLP is exploited to learn the implicit video function. We can observe from Ex. 4 that the MLP layer can improve the performance by 0.16 dB in PSNR and 0.0028 in SSIM.

First, we try to remove the DAM and replace with two other fusion mechanisms: (Ex. 1) single feature path that directly receives the concatenated blurry image and its event frames, (Ex. 3) dual feature path that concatenates after extracting features from blurry image and event frames separately. These two methods can be regarded as the pre-fusion and post-fusion respectively. Compared to them, our method utilize the DAM to take the complementary merits of frames and events, where a bidirectional enhancement process is implemented to suppress the noise in event features and simultaneously deblur image features, and thus improve the performance by a large margin (0.825dB in PSNR and 0.0173 in SSIM). Moreover, we found that pre-fusion by concatenation of two information sources performs better than the model with only a dual feature path, where the mutual compensation of dual features is not fully explored. This further proves the importance of DAM in our DFEN in terms of motion deblurring. In our method, the continuous-time decoding MLP is the crucial module to learn the implicit video function. The deletion of this module (Ex. 4) makes our method degenerate into a sequence restoration model and slightly reduces the performance (0.16dB in PSNR and 0.0028 in SSIM). The EER module is designed to supplement the lost information among the event frames and refine the detailed textures. The comparison of Ex. 5 and Ex. 6 (or Ex. 2 and Ex. 3) validate its effectiveness.

\noindent\textbf{Noise Suppression} 
To further verify the effectiveness of DAM in noise suppression, we evaluate our model (with DAM) and the model without DAM, \ie, Ex. 3 in \cref{tab:ablation}, on the REDS dataset that is contaminated by noisy events generated from the uniform random distribution as \cite{wang2020event}. 
In \cref{tab:noise}, we compare the performance of the above two models under different noise levels ranging from 0\% to 30\%, where the noise level is defined as the proportion of noisy events to the original events. In the cases of no or low noise (0\% and 5\%), the model with DAM already outperforms its counterpart by a large margin, benefiting from the mutual compensation of image and event features in DAM. As the noise level rises, the performance gap becomes more evident since our network can exploit the smooth image features to enhance the information in event features while suppressing noise.  

% showing that DAM plays a role in noise suppression.

% As shown in \cref{tab:noise}, we evaluate the performance changes of both networks under different level of event noise.
% Event-based deblurri  ng method relies on high-quality events, naturally, with the increasing proportion of event noise, the process of deblurring will be seriously affected and the performance shows a downward trend for both networks.
% However, it can see that the trend of network performance decreasing with increasing noise ratio becomes slower for our network comparing to another one, which shows that DAM plays a role in noise suppression.

% The dual attention mechanism is used for mutual compensation between the blurry image and events, including a bidirectional enhancement, \ie, E2B and B2E. 
% To validate their effectiveness, four experiments (Ex. 4-6 and 8) have been carried out. It is shown that B2E and E2B respectively bring PSNR gain of 0.58 dB and {0.861 dB}. While combining B2E and E2B can achieve further improvement (1.014 dB in PSNR) which validates the importance of the dual attention mechanism.

% \par
% \noindent\textbf{MLP.} In DeMo-IVF, MLP is exploited to learn the implicit video function. We can observe from Ex. 7 that the MLP layer can improve the performance by 0.292 dB in PSNR.

In addition to quantitative comparisons, the qualitative results are depicted in \cref{fig:noise}.
In the noise-free scenarios, the networks with and without DAM are both able to remove motion blurs and restore sharp images by utilizing high-quality event streams. However, with the surge in the noise level, the model without DAM is severely disturbed by event noise, leading to noisy textures and unpleasant visual effects.
% It can be seen that, without adding event noise, both networks can utilize the high-quality event stream to remove motion blur and restore sharp images.
% With the increased proportion of event noise, the network without DAM is severely affected by that and produce outputs with much noise and artifacts. 
By utilizing the less noisy image features, DFEN mitigates the disturbance and produces smoother and more realistic textures, which further illustrates the importance of DAM for event noise suppression.

\noindent\textbf{Training Strategy}
% To alleviate the bias issue caused by sparse sampling, we apply the flow loss $\mathcal{L}_{flow}$ to supervise the restoration of frames without references. 
Our training process is divided into two steps: (1) optimize the DFEN and MLP with $\mathcal{L}_{im}$ and $\mathcal{L}_{motion}$, (2) optimize EER with $\mathcal{L}_{refine}$. In this section, we present investigations on ablation of the loss function in each step.
% For training strategy, $L_{im}$, $L_{motion}$ and $L_{EER}$ are used to optimize the model. To verify their effects, the ablation experiments is conducted on the REDS dataset. 
The results are shown in \cref{tab:reds_flow_er} and \cref{fig:ablation_flow_er}. 
% 分析实验结果

% A 仅使用key监督训练的结果
First, only the $\mathcal{L}_{im}$ loss is applied for supervision (Ex. A). As might have been expected, the model only reconstructs sharp images at the referenced timestamps, but performs poorly at non-referenced timestamps, where its reconstructions exhibit severe ghosting artifacts and look like the overlay of the two adjacent sharp frames at reference timestamps. This indicates that the sparse sampling in $\mathcal{L}_{im}$ loss will bias the network towards learning to reconstruct sharp images at the timestamps with references.

% B 同时使用key监督和flow loss的结果
When the $\mathcal{L}_{motion}$ loss is also included (Ex. C), the network learn to make temporally continuous reconstruction, alleviating the bias issue. The model predicts sharp images at both reference and non-reference timestamps and achieves a large performance increment (2.955dB in PSNR and 0.0998 in SSIM). Nevertheless, it can be observed that the reconstructed images have slight artifacts and noise in this condition. The reconstruction quality on reference timestamp even drops compared to Ex.A. This is because the error introduced by the estimated optical flow will lead to performance degradation.

% C EER
The EER and $\mathcal{L}_{refine}$ is just designed to tackle this problem. As we further add EER module (Ex. D), the performance is improved again (1.16dB in PSNR and 0.022 in SSIM) with clearer reconstructions and finer details. In addition, we also try to add EER on the basis of Ex.A (Ex. B). In this case, EER still bring some performance improvement (0.798dB in PSNR and 0.0262 in SSIM). Despite that, the EER module still can not repair the serious artifacts at the non-reference timestamps, which illustrate the necessity of $\mathcal{L}_{motion}$ as well.
% Although this method might be limited by the accuracy of the predicted optical flow, 
% It is shown in \cref{fig:flow_loss} that the additional photometric supervision can effectively boost the restoration performance.
% To alleviate the bias issue caused by sparsely sampling, the data warped from gt by pseudo flow are used to supervise the prediction at randomly sampled time. 

% \section{Limitations}
% The principle of the DeMo-IVF is employing events to mitigate the burden of motion ambiguity caused by blurry artifacts. Thus, its performance largely relies on the quality of events.
% On one hand, events triggered under lower illumination experience larger latency due to the intrinsic response time of the photoceceptor \cite{hu2021a}, which brings a burden when apply DeMo-IVF in the dark environment. On the other hand, training the DeMo-IVF-$\infty$ requires an event-based OF prediction network for the flow consistency, thus the performance can be further improved if the OF can be accurately provided.


%which might limit the performance if OF cannot be accurately given.
%In order to verify the contributions of each module in our network architecture, we compare a few variants with and without dual branch architecture, dual-attention W-MSA blocks, and Time-continuous Decoding MLP, as shown in Tab.~\ref{tab:ablation}. 
%For fair comparison, we train all the variants supervised by 7 sharp images and evaluate the performance on deblurring to reconstruct 7 frames.
%From the table, we can draw the following conclusions:
%Dual-branch architecture can help extract features from event and blur image respectively, and improve the performance with the aid of effective feature fusion module. Comparing the results of 2nd and 5th rows, 3rd and 6th rows, it can be seen that using dual branch architecture can improve PSNR by about 0.4 dB with the aid of dual-attention W-MSA blocks. Comparing the 1st and 4th rows, we can see that without effective fusion module, the use of dual branch architecture will lead to the decline of performance instead, which also proves the effectiveness of dual-attention W-MSA blocks on mutual enhancement between event feature and image feature. In addition, the results of 1st and 3rd rows show that the W-MSA blocks can also help extract features better.
%The time-continuous decoding module is mainly used to decode corresponding latent sharp images given the encoded time from the extracted features. From 2nd and 3rd rows, 5th and 6th rows, we can see that this module can improve performance slightly in dual-branch architecture and kill performance in single-branch architecture.

% \paragraph{validation of attention map or visual ablation study of model}
% it is to show the effectiveness of transformer, three transformer attention maps should be shown\\
% 1. add noise to events\\
% 2. without E to B concat, show attention map \\
% 3. without B to E attention, show attention map \\
% 3. with both of them, show attention map \\


% \paragraph{qualitative results of training with optical flow}



% \paragraph{with respect to different position encoding length on $t$}

% \paragraph{with respect to supervision frames 3-5-7}



==> sec/5_conclusions.tex <==
\section{Conclusion}
This paper proposes a novel DeMo-IVF method to fully demystify motion blurred observations by learning an implicit video function from blurry images and the concurrent event streams. 
Different from existing deblurring methods, our proposed DeMo-IVF is able to query the latent sharp images at arbitrary time instances within the exposure period of blurry inputs. In addition, a dual feature embedding network is proposed to make full use of frames and events, simultaneously achieving blurry feature enhancement and event noise suppression.
% mutual compensation of cross-modal signals.
Extensive experiments on both synthetic and real-world datasets demonstrate that our DeMo-IVF achieves state-of-the-art deblurring performance and fully recovers the scene dynamics behind blurry images.

% shows advantages in temporal resolution. 

% on both synthetic and real-world scenarios.

==> useless/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> useless/fig_reds_31.tex <==
\def\spymag{3.3} % 放大倍数
\def\spysize{0.7cm} %小方框的size
\def\spyheight{1.43cm}
\def\spywidth{2.53cm}
\def\spysmallpos{( 0.86,  0.48)} %小方框的位置
\def\spylargepos{( 0, -0.75)} %大方框位置

\def\subwidth{0.14\textwidth} %子图大小
\def\subsep{-1.6mm}           %子图间距
\renewcommand{\imgfont}{\fontsize{7}{6}\selectfont}
\begin{figure*}[!thb]
	\centering
    % LEDVDI
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/LEDVDI_003_00.png}}; 
            \spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
            \node (RED) [align=center, draw=none, rotate=90, font=\imgfont] at (-1.4, -0.8) {\textcolor{black}{LEDVDI + Timelens}};
	\end{tikzpicture} 
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/LEDVDI_003_01.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture}
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/LEDVDI_003_02.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture}
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/LEDVDI_003_03.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture}
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/LEDVDI_003_04.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture}
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/LEDVDI_003_05.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture}
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/LEDVDI_003_06.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture} 

    %
    \begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/RED-Net_003_00.png}}; 
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
            \node (RED) [align=center, draw=none, rotate=90, font=\imgfont] at (-1.4, -0.8) {\textcolor{black}{RED-Net + Timelens}};
        \end{tikzpicture} 
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/RED-Net_003_01.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture}
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/RED-Net_003_02.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture}
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/RED-Net_003_03.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture}
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/RED-Net_003_04.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture}
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/RED-Net_003_05.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture}
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/RED-Net_003_06.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture} 

    % Ours
    \begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/ours_003_00.png}}; 
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
            \node (RED) [align=center, draw=none, rotate=90, font=\imgfont] at (-1.4, -0.8) {\textcolor{black}{Ours}};
	\end{tikzpicture} 
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/ours_003_01.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture}
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/ours_003_02.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture}
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/ours_003_03.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture}
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/ours_003_04.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture}
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/ours_003_05.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture}
        \hspace{\subsep}
	\begin{tikzpicture}[spy using outlines={green,magnification=\spymag,height=\spyheight,width=\spywidth},inner sep=0]
		\node {\includegraphics[width=\subwidth]{fig/fig_REDS_31/ours_003_06.png}};
  		\spy on \spysmallpos in node [below, line width=0.5pt] at \spylargepos;
	\end{tikzpicture} 


	\caption{
            Qualitative comparisons of the sequence restoration where $31$ latent frames are restored from one single blurry image on the REDS dataset: RED-Net (+ Interpolation), LEDVDI (+ Interpolation), and our method. Only the first $7$ consecutive images of the entire sequence are shown here.}
	\label{fig:reds_31}
 % \vspace{-1em}
\end{figure*}
